Generalizing to Unseen Domains: A Survey on Domain Generalization

Machine learning systems generally assume that the training and testing distributions are the same. To this end, a key requirement is to develop models that can generalize to unseen distributions. Domain generalization (DG), i.e., out-of-distribution generalization, has attracted increasing interests in recent years. Domain generalization deals with a challenging setting where one or several different but related domain(s) are given, and the goal is to learn a model that can generalize to an unseen test domain. Great progress has been made in the area of domain generalization for years. This paper presents the first review of recent advances in this area. First, we provide a formal definition of domain generalization and discuss several related fields. We then thoroughly review the theories related to domain generalization and carefully analyze the theory behind generalization. We categorize recent algorithms into three classes: data manipulation, representation learning, and learning strategy, and present several popular algorithms in detail for each category. Third, we introduce the commonly used datasets, applications, and our open-sourced codebase for fair evaluation. Finally, we summarize existing literature and present some potential research topics for the future.

==> DG survey -- TKDE/figures/fig-application.tex <==
% \begin{forest}
%   for tree={
%   grow=east,
%   reversed=true,
%   anchor=base west,
%   parent anchor=east,
%   child anchor=west,
%   base=left,
%   font=\small,
%   rectangle,
%   draw,
%   rounded corners,align=left,
%   minimum width=2.5em,
%   inner xsep=4pt,
%   inner ysep=1pt,
%   },
%   where level=1{text width=5em,fill=blue!10}{},
%   where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
%   where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
%   [Domain\\generalization\\applications,fill=green!20
%     [Computer\\vision,text width=5em
%         [Image classification,text width=8em
%             % [e.g. \cite{yue2019domain,li2017deeper,liu2021learning}
%             % ]
%         ]
%         % [Semantic segmentation,text width=9em
%         %   [e.g. \cite{gong2019dlow,li2021semantic}
%         %   ]
%         % ]
%         % [Action recognition,text width=8em
%         %     [e.g. \cite{li2017domain,li2019episodic}
%         %     ]
%         % ]
%         % [Person Re-ID,text width=6em
%         %     [e.g. \cite{wang2020domainmix,jin2020feature}
%         %     ]
%         % ]
%     ]
%         % [Natural\\language\\processing,text width=5em
%         %     [Sentiment classification,text width=9em
%         %         [e.g. \cite{wang2020unseen,balaji2018metareg}
%         %         ]
%         %     ]
%         %     [Semantic parsing,text width=7em
%         %      [e.g. \cite{wang2020meta}
%         %      ]
%         %     ]
%         %     [Web page classification,text width=9em
%         %         [e.g. \cite{garg2020learn}
%         %         ]
%         %     ]
%         % ]
%         % [Reinforcement\\learning,text width=6em
%         %     [Robot control,text width=5em
%         %         [e.g. \cite{li2018learning2,zhoudomain}
%         %         ]
%         %     ]
            
%         % ]
%         % [Medical\\analysis,text width=5em
%         %     [Tissue segmentation,text width=8em
%         %         [e.g. \cite{Dou2019DomainGV}
%         %         ]
%         %     ]
%         %     [Parkinson's disease,text width=8em
%         %         [e.g. \cite{muandet2013domain}
%         %         ]
%         %     ]
%         %     [Chest X-ray recognition,text width=9em
%         %         [e.g. \cite{Mahajan2020DomainGU,li2020domain}
%         %         ]
%         %     ]
%         %     [EEG-based seizure detection,text width=11em
%         %         [e.g. \cite{ayodele2020supervised}
%         %         ]
%         %     ]
%         % ]
%         % [Other\\applications,text width=5em
%         %     [Human activity recognition,text width=11em
%         %         [e.g. \cite{qian2021latent}
%         %         ]
%         %     ]
%         %     [Fault diagnosis,text width=6em
%         %         [e.g. \cite{li2020domain,liao2020deep,zheng2020deep}
%         %         ]
%         %     ]
%         %     [Time series forecasting,text width=9em
%         %         [e.g. \cite{du2021adarnn}
%         %         ]
%         %     ]
%         %     [Speech utterance recognition,text width=11em
%         %         [e.g. \cite{shankar2018generalizing,piratla2020efficient}
%         %         ]
%         %     ]
%         % ]
%     ]
% \end{forest}

\begin{forest}
  for tree={
  grow=east,
  reversed=true,
  anchor=base west,
  parent anchor=east,
  child anchor=west,
  base=left,
  font=\small,
  rectangle,
  draw,
  rounded corners,align=left,
  minimum width=2.5em,
  inner xsep=4pt,
  inner ysep=1pt,
  },
  where level=1{text width=5em,fill=blue!10}{},
  where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
  where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
  [Domain\\generalization\\applications,fill=green!20
    [Computer\\vision,text width=4.5em
        [Image classification,text width=7.5em
            [e.g. DRPC \cite{yue2019domain}/ CSG \cite{liu2021learning}
            ]
        ]
        [Semantic segmentation,text width=9em
          [e.g. DLOW \cite{gong2019dlow}/ \cite{li2021semantic}
          ]
        ]
        [Action recognition,text width=8em
            [e.g. Epi-FCR \cite{li2019episodic}/ \cite{li2017domain}
            ]
        ]
        [Person Re-ID,text width=5.5em
            [e.g. DomainMix \cite{wang2020domainmix}/ FAR \cite{jin2020feature}
            ]
        ]
    ]
    [Natural\\language\\processing,text width=5em
        [Sentiment classification,text width=9em
            [e.g. MetaReg \cite{balaji2018metareg}/ \cite{wang2020unseen}
            ]
        ]
        [Semantic parsing,text width=7em
         [e.g. \cite{wang2020meta}
         ]
        ]
        [Web page classification,text width=9em
            [e.g. FSUS \cite{garg2020learn}
            ]
        ]
    ]
    [Reinforcement\\learning,text width=6em
        [Robot control,text width=5em
            [e.g. MLDG \cite{li2018learning2}/ MixStyle \cite{zhoudomain}
            ]
        ]
    ]
    [Medical\\analysis,text width=5em
        [Tissue segmentation,text width=8em
            [e.g. MASF \cite{Dou2019DomainGV}
            ]
        ]
        [Parkinson's disease,text width=8em
            [e.g. DICA \cite{muandet2013domain}
            ]
        ]
        [Chest X-ray recognition,text width=9em
            [e.g. MatchDG \cite{Mahajan2020DomainGU}/ \cite{li2020domain}
            ]
        ]
        [EEG-based seizure detection,text width=11em
            [e.g. \cite{ayodele2020supervised}
            ]
        ]
    ]
    [Other\\applications,text width=5em
        [Human activity recognition,text width=10.5em
            [e.g. GILE \cite{qian2021latent}/ LAG \cite{lu2022local}
            ]
        ]
        [Fault diagnosis,text width=6em
            [e.g. DSDGN \cite{liao2020deep}/ DDGFD \cite{zheng2020deep}/ \cite{li2020domain}
            ]
        ]
        [Time series forecasting,text width=9em
            [e.g. AdaRNN \cite{du2021adarnn}
            ]
        ]
        [Speech utterance recognition,text width=10.8em
            [e.g. CrossGrad \cite{shankar2018generalizing}/CSD \cite{piratla2020efficient}
            ]
        ]
    ]
]
\end{forest}

        

==> DG survey -- TKDE/figures/fig_tree.tex <==
\begin{forest}
  for tree={
  grow=east,
  reversed=true,
  anchor=base west,
  parent anchor=east,
  child anchor=west,
  base=left,
  font=\small,
  rectangle,
  draw,
  rounded corners,align=left,
  minimum width=2.5em,
  inner xsep=4pt,
  inner ysep=1pt,
  },
  where level=1{text width=5em,fill=blue!10}{},
  where level=2{text width=5em,font=\footnotesize,fill=pink!30}{},
  where level=3{font=\footnotesize,yshift=0.26pt,fill=yellow!20}{},
  [Domain \\ generalization\\algorithms,fill=green!20
        [Data\\manipulation\\(Sec.~\ref{sec-method-data}),text width=6em
            [Data augmentation,text width=8em
              [\emph{Domain randomization:} DRPC \cite{yue2019domain}/ SDR \cite{prakash2019structured}/ FSDR \cite{huang2021fsdr}/ \cite{tobin2017domain,peng2018sim,khirodkar2019domain,tremblay2018training,nazari2020domain}
              ]
              [\emph{Adversarial data augmentation:} CrossGrad \cite{shankar2018generalizing}/ ADA \cite{volpi2018generalizing}/ DDAIG \cite{zhou2020deep}
              ]
            ]
            [Data generation,text width=7em [M-ADA \cite{qiao2020learning}/ UFDN \cite{liu2018unified}/ UNVP \cite{truong2019recognition}/ L2A-OT \cite{Zhou2020LearningTG}/ M3L \cite{zhao2020learning}/  FSUS \cite{garg2020learn}/ ADAGE \cite{maria2019hallucinating}/ \\ DomainMix \cite{wang2020domainmix}/ MixALL \cite{wang2020heterogeneous}/ MixStyle \cite{zhoudomain}/ DeGIA \cite{truong2019image}/  MBDG \cite{robey2021model}/ PDEN \cite{li2021progressive}/ \\ SFA \cite{li2021simple}/ OpenDG \cite{shu2021open}/  FACT \cite{xu2021fourier}/ \cite{rahman2019multi,somavarapu2020frustratingly,nazari2020domain,peng2021out,wang2021learningtodiversify}
              ]
            ]
        ]
        [Representation\\learning\\(Sec.~\ref{sec-repr}),text width=6em
          [Domain-invariant\\representation learning,text width=8.5em
              [\emph{Kernel methods:} MTL \cite{blanchard2011generalizing,blanchard2017domain}/ Multi-TCA \cite{grubinger2015domain}/ DICA \cite{muandet2013domain}/ UDICA \cite{gan2016learning}/ CIDG \cite{li2018domain}/ SCA \cite{ghifary2016scatter}/ \\ ESRand \cite{erfani2016robust}/ MDA \cite{hu2019domain}/ \cite{deshmukh2019generalization}
              ]
              [\emph{Explicit feature alignment:} MTAE \cite{Ghifary2015DomainGF}/ CCSA \cite{motiian2017unified}/ BNE \cite{segu2020batch}/ SNR \cite{jin2020style,jin2021style}/ MMD-AAE \cite{Li2018DomainGW}/ \\ DDGFD \cite{zheng2020deep}/ DSDGN \cite{liao2020deep}/  DG-YOLO \cite{liu2020towards}/ MatchDG \cite{Mahajan2020DomainGU}/  DSON \cite{seo2020learning}/  DFDG \cite{zhang2021robust}/ DSAF \cite{qi2021unsupervised}/ \\ AdaRNN \cite{du2021adarnn}/ ASR-Norm \cite{fan2021adversarially}/ RNA-Net \cite{planamente2021domain}/ FAR \cite{jin2020feature}/ LAG \cite{lu2022local}/ \cite{maniyar2020zero,han2020domain,gulrajani2021search,ayodele2020supervised,chen2020study,li2020domain}
              ]
              [\emph{Domain adversarial learning:} DANN \cite{ganin2015unsupervised,Ganin2016DomainAdversarialTO}/ MMD-AAE \cite{Li2018DomainGW}/ DLOW \cite{gong2019dlow}/ CIAN \cite{li2018deep}/ ER \cite{zhao2020domain}/ \\ MADDG \cite{shao2019multi}/  FSUS \cite{garg2020learn}/ MMLD \cite{Matsuura2020DomainGU}/ DANNCE \cite{sicilia2021domain}/ CAADG \cite{rahman2020correlation}/ SSDG \cite{jia2020single}/ AdaRNN \cite{du2021adarnn} \\ ASR-Norm \cite{fan2021adversarially}/ SADG \cite{luo2021scale}/ \cite{albuquerque2019adversarial,wang2020unseen}
              ]
              [\emph{Invariant risk minimization:} IRM \cite{arjovsky2019invariant}/IB-IRM \cite{ahuja2021invariance}/VRex \cite{krueger2021out}/ReLIC \cite{mitrovic2021representation}/\cite{guo2021out,ahuja2020empirical,choe2020empirical,rosenfeld2020risks,pmlr-v119-ahuja20a}
              ]
          ]
          [Feature disentanglement, text width=9.5em
            [\emph{Multi-component analysis:} LRE-SVM \cite{xu2014exploiting,li2017domain}/ UndoBias \cite{khosla2012undoing}/ MVDG \cite{niu2015multi}/ CSD \cite{piratla2020efficient}/ \\ Domain2Vec \cite{deshmukh2018domain2vec,peng2020domain2vec}/   DCAC \cite{hu2021domain}/ FLUTE \cite{triantafillou2021learning}/  \cite{ding2017deep,li2017deeper,zunino2020explainable}
            ]
            [\emph{Generative modeling:} DIVA \cite{ilse2019diva}/ DAL \cite{peng2019domain}/ M-ADA \cite{qiao2020learning}/ DDG \cite{zhang2021towards}/ SagNet \cite{nam2021reducing}/ GILE \cite{qian2021latent} \\ RobustNet \cite{choi2021robustnet}/ \cite{li2021semantic}
            ]
            [\emph{Causality-inspired methods:} MatchDG \cite{Mahajan2020DomainGU}/ Deep CAMA \cite{zhang2020causal}/ CSG \cite{liu2021learning}/  LaCIM \cite{sun2021recovering}/ \\ StableNet \cite{zhang2021deep}/ \cite{mitrovic2021representation,ouyang2021causality,he2019towards}
            ]
          ]
        ]
        [Learning\\strategy\\(Sec.~\ref{sec-method-learn}),text width=6em
          [Ensemble learning,text width=7em
            [D-SAM \cite{d2018domain}/ DAEL \cite{zhou2020domain}/ COPA \cite{wu2021collaborative}/ \cite{mancini2018best,he2018domain,mancini2018robust,dubey2021adaptive}]
            ]
          [Meta-learning, text width=6em
            [MLDG \cite{li2018learning2}/ MetaReg \cite{balaji2018metareg}/ FC \cite{li2019feature}/ MASF \cite{Dou2019DomainGV}/ MetaVIB \cite{Du2020LearningTL}/ DADG \cite{chen2020discriminative}/ DGSML \cite{sharifi2020domain}/ M3L \cite{zhao2020learning}/ \\ Epi-FCR \cite{li2019episodic}/ \cite{wang2020meta,qiao2021uncertainty,kim2021self}]
            ]
         [Gradient operation, text width=8em
            [RSC \cite{huang2020self}/ Fish \cite{shi2021gradient}/ Fishr \cite{rame2021fishr}/ NCDG \cite{tian2021neuron}/ KDDG \cite{wang2021embracing}]
            ]
         [Distributionally robust optimization, text width=14em
            [VRex \cite{krueger2021out}/ JTT \cite{liu2021just}/ GroupDRO \cite{sagawa2019distributionally}/ \cite{koh2020wilds,wang2021class}]
            ]
         [Self-supervised learning, text width=9em
            [JiGen \cite{carlucci2019domain}/ SelfReg \cite{kim2021selfreg}/ \cite{jeon2021feature,li2021domain}]
            ]
          [Others, text width=2.5em
                [Random forest~\cite{ryu2019generalized}/Shape-invariant~\cite{narayanan2021shape}/Lottery ticket hypothesis~\cite{zhang2021can}/Flat minima~\cite{cha2021swad}/
                Metric learning~\cite{faraki2021cross}
                ]
            ]
        ]
    ]
\end{forest}

==> DG survey -- TKDE/secs/sec_application.tex <==
% \section{Applications}
% \label{sec-app}
In this section, we discuss the popular tasks/applications for \dg (ref. \figurename~\ref{fig-app}).


%In this section, we discuss popular applications for \dg.
%While most of the literature utilized image classification as the main benchmark application (refer to the datasets in previous section), there are other areas where DG also plays a key role.

High generalization ability is desired in various vision tasks. Many works investigate DG on classification. Some works also study DG for semantic segmentation~\cite{gong2019dlow}, action recognition~\cite{li2017domain,li2019episodic}, face anti-spoofing~\cite{shao2019multi}, person Re-ID~\cite{wang2020domainmix,jin2020feature}, street view recognition~\cite{qiao2020learning}, video understanding~\cite{niu2015multi}, and image compression~\cite{zhang2021out}.
Medical analysis~\cite{hu2021domain} is one of the important application areas for DG due to its nature of data scarcity and existence of domain gaps, with the tasks of tissue segmentation~\cite{Dou2019DomainGV}, Parkinson's disease recognition~\cite{muandet2013domain}, activity recognition~\cite{erfani2016robust}, chest X-ray recognition~\cite{Mahajan2020DomainGU,li2020domain}, and EEG-based seizure detection~\cite{ayodele2020supervised}. 

Apart from those areas, DG is also useful in reinforcement learning of robot control~\cite{zhoudomain,li2018learning2} to generalize to an unseen environment.
Some work used DG to recognize speech utterance~\cite{shankar2018generalizing,piratla2020efficient}, fault diagnosis~\cite{li2020domain,liao2020deep,zheng2020deep}, physics~\cite{chen2020study}, brain-computer interface~\cite{han2020domain}.

\begin{figure}[t!]
	\centering
	\resizebox{.5\textwidth}{!}{
	\input{figures/fig-application}
	}
	\caption{Several applications of \dg.}
	\label{fig-app}
\end{figure}

% While most of the literature utilized image classification as the main benchmark application (refer to the datasets in previous section), there are other areas where DG also plays a key role.

% In computer vision, apart from image classification, satellite image classification~\cite{deshmukh2019generalization} is also a popular application for DG.
% Some works also used DG for semantic segmentation~\cite{gong2019dlow}, action recognition~\cite{li2017domain,li2019episodic}, face anti-spoofing~\cite{shao2019multi}, person Re-ID~\cite{wang2020domainmix,jin2020feature}, and street view recognition~\cite{qiao2020learning}.
% Also, there are some work for video understanding~\cite{niu2015multi}, and hand pose recognition~\cite{truong2019image}.
% In these applications, there are also some training domains with different distributions where DG is used to learn general and robust representations.

In natural language processing, it is also common that training data comes from different domains with different distributions and DG techniques are helpful. 
Some work used \dg for sentiment classification on the Amazon Review dataset~\cite{wang2020unseen,balaji2018metareg}.
Others used DG for semantic parsing~\cite{wang2020meta}, web page classification~\cite{garg2020learn}. For instance, if we are given natural language data from multiple domains and want to learn a generalized model that predicts well on any new domain, we can use \dg to acquire domain-invariant representations.

Moreover, DG techniques favor broad prospects in some applications, such as financial analysis, weather prediction, and logistics.
For instance, \citet{du2021adarnn} tried to adopt DG to time series modeling. They first propose the temporal covariate shift problem that widely exists in time series data, then, they proposed an RNN-based model to solve this problem to align the hidden representations between any pair of training data that are from different domains.
Their algorithm, the so-called AdaRNN, was applied to stock price prediction, weather prediction, and electric power consumption.
Another example is \cite{qian2021latent}, where they applied domain generalization to sensor-based human activity recognition.
In their application, the activity data from different persons are from different distributions, resulting in severe model collapse when applied to new users.
To resolve such problem, they developed a variational autoencoder-based network to learn the domain-invariant and domain-specific modules, thus achieving the disentanglement.

In the future, we hope there can be more DG applications in other areas to tackle with the distributional shift that widely exists in different applications.
Another important problem is the evaluation of DG algorithms without accessing the test distribution in reality. While we can use the test data for evaluation in research, we simply cannot do it for real applications. In this case, one possible approach would be performing meta-train and meta-test split for the original data for multiple times. In each time, one split can be regarded as the unseen test data while the other as the training data. We can call it the meta-cross-validation for DG in reality. At the same time, we also hope there could be more evaluation metrics. For more evaluation in research, please refer to the next section.


==> DG survey -- TKDE/secs/sec_application_V1.0-old.tex <==
% \section{Applications}
% \label{sec-app}
In this section, we discuss popular applications for \dg.
While most of the literature utilized image classification as the main benchmark application (refer to the datasets in previous section), there are other areas where DG also plays a key role.

In computer vision, apart from image classification, satellite image classification~\cite{deshmukh2019generalization} is also a popular application for DG.
Some works also used DG for semantic segmentation~\cite{gong2019dlow}, action recognition~\cite{li2017domain,li2019episodic}, face anti-spoofing~\cite{shao2019multi}, person Re-ID~\cite{wang2020domainmix,jin2020feature}, and street view recognition~\cite{qiao2020learning}.
Also, there are some work for video understanding~\cite{niu2015multi}, and hand pose recognition~\cite{truong2019image}.
In these applications, there are also some training domains with different distributions where DG is used to learn general and robust representations.

In natural language processing, it is also common that training data comes from different domains with different distributions. 
Some work used \dg for sentiment classification on the Amazon Review dataset~\cite{wang2020unseen,balaji2018metareg}.
Others used DG for semantic parsing~\cite{wang2020meta}, web page classification~\cite{garg2020learn}.

Medical analysis is one of the key application areas for DG due to its nature of data scarcity.
In this field, tissue segmentation~\cite{Dou2019DomainGV}, Parkinson's disease~\cite{muandet2013domain}, activity recognition~\cite{erfani2016robust}, tissue segmentation~\cite{Dou2019DomainGV}, chest X-ray recognition~\cite{Mahajan2020DomainGU,li2020domain}, and EEG-based seizure detection~\cite{ayodele2020supervised}. 

Apart from those areas, DG was also used in reinforcement learning of robot control~\cite{zhoudomain,li2018learning2} to generalize to unseen environment.
Some work used DG to recognition speech utterance~\cite{shankar2018generalizing,piratla2020efficient}, fault diagnosis~\cite{li2020domain,liao2020deep,zheng2020deep}, physics~\cite{chen2020study}, brain-computer interface~\cite{han2020domain}.

Nowadays, there is a growing interest to apply existing machine learning techniques to different applications, such as financial analysis, stock prediction, weather prediction, as well as logistics.
Domain generalization is a very fundamental technology that can generally be applied to these and other areas for better generalization performance in new domains.


==> DG survey -- TKDE/secs/sec_biography.tex <==
\begin{IEEEbiography}	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/jindwang.jpg}}]{Jindong Wang} is currently a researcher at Microsoft Research Asia, Beijing, China. He received his Ph.D. degree from Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China, in 2019. He was a visiting student in Hong Kong University of Science and Technology (HKUST) in 2018. His research interest mainly includes transfer learning, machine learning, data mining, and ubiquitous computing. He serves as the publicity co-chair of IJCAI’19 and session chair of ICDM’19. He is the reviewer or PC member of several leading journals and conferences such as TPAMI, TKDE, ICLR, ICML, NeurIPS, CVPR, etc.
\end{IEEEbiography}

\begin{IEEEbiography}	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/Cuiling_Lan.jpg}}]{Cuiling Lan} received the B.S. degree in electrical engineering and the Ph.D. degree in intelligent information processing from Xidian University, Xi’an, China, in 2008 and 2014, respectively. She joined Microsoft Research Asia, Beijing, China, in 2014. Her current research interests include computer vision problems related to pose estimation, action recognition, person/vehicle re-identification, domain generalization/adaptation.
\end{IEEEbiography}
\vspace{-3em}

\begin{IEEEbiography}	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/ChangLiu-1}}]{Chang Liu}
is currently a researcher at Microsoft Research Asia, Machine Learning Group, starting from 2019. Before that, he received his Ph.D. degree in 2019 at the Department of Computer Science and Technology, Tsinghua University. His research interests include general Bayesian inference methods (e.g., variational inference, MCMC), Bayesian and generative modeling, and causal machine learning.

\end{IEEEbiography}
\vspace{-3em}

\begin{IEEEbiography}	[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{figures/figures_bios/yidongouyang.jpg}}]{Yidong Ouyang} is a Ph.D student in School of Data Science, Chinese University of Hong Kong, Shenzhen. His research interests include the generalization and robustness of machine learning.
\end{IEEEbiography}
\vspace{-3em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/taoqin}}]{Tao Qin}
received the Ph.D. degree and Bachelor
degree both from Tsinghua University. He is a Senior
member of ACM and IEEE, and an Adjunct Professor (Ph.D. advisor) in the University of Science
and Technology of China. He is a Senior Principal
Researcher and managing the Deep and Reinforcement Group in Microsoft Research Asia. His research interests include
machine learning (with the focus on deep learning and
reinforcement learning), artificial intelligence (with
applications to language understanding and computer
vision), game theory and multi-agent systems (with
applications to cloud computing, online and mobile advertising, ecommerce),
information retrieval and computational advertising.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/bio-wanglu}}]{Wang Lu}
received the B.S. degree in Mathematics and Applied Mathematics from Tsinghua University, Beijing, China, in 2012 and 2016, and is currently a Ph.D. candidate of the Research Center for Ubiquitous Computing Systems (CUbiCS) at the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS). His research interests include transfer learning, federated learning and activity recognition.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/yqchen.jpg}}]{Yiqiang Chen}
received the B.S. and M.S. degrees in computer science from Xiangtan University, Xiangtan, China, in 1996 and 1999, respectively, and the Ph.D. degree in computer science from the Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China, in 2003. In 2004, he was a Visiting Scholar Researcher with the Department of Computer Science, Hong Kong University of Science and Technology (HKUST), Hong Kong. He is currently a professor and the director of the Pervasive Computing Research Center at the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS). His research interests include artificial intelligence, pervasive computing, and human-computer interaction.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/Wenjun_Zeng.jpg}}]{Wenjun (Kevin) Zeng} is a Sr. Principal Research Manager and a member of the senior leadership team at Microsoft Research Asia. He was with Univ. of Missouri from 2003 to 2016, most recently as a Full Professor. Prior to that, he worked for PacketVideo Corp., Sharp Labs of America, Bell Labs, and Panasonic Technology. Wenjun has contributed significantly to the development of international standards (ISO MPEG, JPEG2000, and OMA). He received his B.E., M.S., and Ph.D. degrees from Tsinghua Univ., the Univ. of Notre Dame, and Princeton Univ., respectively. His current research interests include mobile-cloud media computing, computer vision, and multimedia communications and security.	
He is on the Editorial Board of IJCV. He was an AE of IEEE TCSVT, IEEE Trans. on Info. Forensics \& Security, and IEEE Trans. on Multimedia (TMM). He was on the Steering Committee of IEEE Trans. on Mobile Computing and IEEE TMM. He served as the Steering Committee Chair of IEEE ICME in 2010 and 2011, and has served as the General Chair or TPC Chair for several IEEE conferences ({\it e.g.}, ICME’18, ICIP’17). He was the recipient of several best paper awards. He is a Fellow of the IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/psyu.jpg}}]{Philip S. Yu} received the BS degree in electrical engineering from National Taiwan University, the MS and PhD degrees in electrical engineering from Stanford University, and the MBA degree from New York University. He is a distinguished professor in computer science with the University of Illinois at Chicago and also holds the Wexler chair in information technology. His research interests include big data, including data mining, data stream, database, and privacy. He has published more than 1,000 papers in refereed journals and conferences. He holds or has applied for more than 300 US patents. He is the recipient of the ACM SIGKDD 2016 Innovation Award for his influential research and scientific contributions on mining, fusion, and anonymization of big data, the IEEE Computer Society's 2013 Technical Achievement Award for pioneering and fundamentally innovative contributions to the scalable indexing, querying, searching, mining, and anonymization of big data, and the Research Contributions Award from IEEE ICDM in 2003 for his pioneering contributions to the field of data mining. He also received the ICDM 2013 10-year Highest-Impact Paper Award, and the EDBT Test of Time Award (2014). He was the editor-in-chief of the ACM Transactions on Knowledge Discovery from Data (2011-2017) and the IEEE Transactions on Knowledge and Data Engineering (2001-2004). He is a fellow of the IEEE and ACM.
\end{IEEEbiography}

==> DG survey -- TKDE/secs/sec_data.tex <==
We are always hungry for more training data in machine learning (ML).
The generalization performance of a ML model often relies on the quantity and diversity of the training data.
Given a limited set of training data, data manipulation is one of the cheapest and simplest way to generate samples so as to enhance the generalization capability of the model.
The main objective for data manipulation-based DG is to increase the diversity of existing training data using different data manipulation methods. At the same time, the data quantity is also increased.
Although the theoretical insight for why data augmentation or generation techniques can enhance the generalization ability of a model, experiments by \citet{adila2021understanding} showed that the model tend to make predictions for both OOD and in-distribution samples based on trivial syntactic heuristics for NLP tasks.

We formulate the general learning objective of data manipulation-based DG as:
%The general learning objective of data manipulation-based DG can be formulated as:
\begin{equation}
    \label{eq-augmentation-all}
    \min_{h} \, \mathbb{E}_{\mathbf{x},y} [ \ell(h(\mathbf{x}),y) ] + \mathbb{E}_{\mathbf{x}^\prime,y} [ \ell(h(\mathbf{x}^\prime),y) ],
\end{equation}
where $\mathbf{x}^\prime = \mathcal{M}(\mathbf{x})$ denotes the manipulated data using a function $\mathcal{M}(\cdot)$.
Based on the difference on this function, we further categorize existing work into two types: \emph{data augmentation} and \emph{data generation}.

\subsubsection{Data augmentation-based DG}
Augmentation is one of the most useful techniques for training machine learning models.
Typical augmentation operations include flipping, rotation, scaling, cropping, adding noise, and so on.
They have been widely used in supervised learning to enhance the generalization performance of a model by reducing overfitting \cite{shorten2019survey,nazari2020domain}.
Without exception, they can also be adopted for DG where $\mathcal{M}(\cdot)$ can be instantiated as these data augmentation functions.
%It is intuitive to introduce them to \dg to enhance the generalization performance of a model, where $\operatorname{mani}$ can be instantiated as some data augmentation functions.
%\tcb{\cite{}}

\paragraph{\textbf{Domain randomization}}
Other than typical augmentation, domain randomization is an effective technique for data augmentation.
It is commonly done by generating new data that can simulate complex environments based on the limited training samples.
Here, the $\mathcal{M}(\cdot)$ function is implemented as several manual transformations (commonly used in image data) such as: altering the location and texture of objects, changing the number and shape of objects, modifying the illumination and camera view, and adding different types of random noise to the data.
\citet{tobin2017domain} first used this method to generate more training data from the simulated environment for generalization in the real environment.
Similar techniques were also used in \cite{peng2018sim,khirodkar2019domain,tremblay2018training,yue2019domain} to strengthen the generalization capability of the models.
\citet{prakash2019structured} further took into account the structure
of the scene when randomly placing objects for data generation, which enables the neural network to learn to utilize context when detecting objects.
\citet{peng2021out} proposed to not only augment features, but also labels.
It is easy to see that by randomization, the diversity of samples can be increased.
But randomization is often random, indicating that there could be some useless randomizations that could be further removed to improve the efficiency of the model.
%

% that has achieved competitive performance

\paragraph{\textbf{Adversarial data augmentation}}
%Domain randomization methods do not explicitly model the information contained in each domain.
%, where the augmentation operations are not guided by optimization objectives.
%While domain randomization methods remain simple and effective for DG, they do not explicitly model the information contained in each domain, thus may lack domain-specific features.
Adversarial data augmentation aims to guide the augmentation to optimize the generalization capability, by enhancing the diversity of data while assuring their reliability. % was proposed to handle this challenge.
\citet{shankar2018generalizing} used a Bayesian network to model dependence between label, domain and input instance, and proposed CrossGrad, a cautious data augmentation strategy that perturbs the input along the direction of greatest domain change while changing the class label as little as possible. 
\citet{volpi2018generalizing} proposed an iterative procedure that augments the source dataset with examples from a fictitious target domain that is ``hard" under the current model, where adversarial examples are appended at each iteration to enable adaptive data augmentation. 
\citet{zhou2020deep} adversarially trained a transformation network for data augmentation instead of directly updating the inputs by gradient ascent while they adopted the regularization of weak and strong augmentation in \cite{zhou2021semi,huang2021fsdr}.
Adversarial data augmentation often has certain optimization goals that can be used by the network.
However, its optimization process often involves adversarial training, thus is difficult.

\subsubsection{Data generation-based DG}
Data generation is also a popular technique to generate diverse and rich data to boost the generalization capability of a model.
Here, the function $\mathcal{M}(\cdot)$ can be implemented using some generative models such as Variational Auto-encoder (VAE)~\cite{kingma2013auto}, and Generative Adversarial Networks (GAN)~\cite{goodfellow2014generative}.
In addition, it can also be implemented using the Mixup~\cite{zhang2018mixup} strategy.

% \paragraph{Data generation using GANs.}
\citet{rahman2019multi} used ComboGAN~\cite{anoosheh2018combogan} to generate new data and then applied domain discrepancy measure such as MMD~\cite{gretton2012kernel} to minimize the distribution divergence between real and generated images to help learn general representations.
\citet{qiao2020learning} leveraged adversarial training to create ``fictitious" yet ``challenging" populations, where a Wasserstein Auto-Encoder (WAE)~\cite{tolstikhin2017wasserstein} was used to help generate samples that preserve the semantic and have large domain transportation.
%relax the widely used worst-case constraint to preserve the semantic and create large domain transportation. 
%Qiao \etal~\cite{qiao2020learning} leveraged adversarial data augmentation by VAEs and explicitly reduce the discrepancy between real and fake images.
% \cl{Liu \etal~\cite{liu2018unified} proposed a Unified Feature Disentanglement Network (UFDN) where they treated both data domains and image attributes of interest as latent factors to be
% disentangled, thus it can be used for domain generation. This work also belongs to the disentanglement category which we will introduce in Section~\ref{sec-repr}. (move to other section)}
\citet{Zhou2020LearningTG} generated novel distributions under semantic consistency and then maximized the difference between source and the novel distributions.
%Zhou \etal \cite{Zhou2020LearningTG} maximized the difference between source and novel distributions and the difference between the generated novel distributions under semantic consistency.
\citet{somavarapu2020frustratingly} introduced a simple transformation based on image stylization to explore cross-source variability for better generalization, where AdaIN \cite{huang2017arbitrary} was employed to achieve fast stylization to arbitrary styles.
Different from others, \citet{li2021progressive} used adversarial training to generate \emph{domains} instead of samples.
These methods are more complex since different generative models are involved and we should pay attention to the model capacity and computing cost.
%Jia \etal~\cite{jia2020single} proposed to generate images and then used adversarial training and triplet loss to regularize the generated images for generalization.
%Some works combined data generation with meta-learning~\cite{zhao2020learning} or Mixed Gaussian distribution~\cite{truong2019recognition}.

% \paragraph{Mixup.}

In addition to the above generative models, Mixup~\citep{zhang2018mixup} is also a popular technique for data generation.
Mixup generates new data by performing linear interpolation between any two instances and between their labels with a weight sampled from a Beta distribution, which does not require to train generative models.
Recently, there are several methods using Mixup for DG, by either performing Mixup in the original space~\citep{wang2020domainmix,wang2020heterogeneous,shu2021open} to generate new samples; or in the feature space~\citep{zhoudomain,qiao2021uncertainty,xu2021fourier} which does not explicitly generate raw training samples.
These methods achieved promising performance on popular benchmarks while remaining conceptually and computationally simple.

==> DG survey -- TKDE/secs/sec_dataset.tex <==
In this section, we summarize the existing common datasets and model selection strategies for \dg.
Then, we introduce the codebase, DeepDG, and demonstrate some observations from experiment conducted via it.

\subsection{Datasets}
% In this section, we introduce the widely used benchmark datasets for \dg.
\tablename~\ref{tb-dataset} offers an overview of several popular datasets.
Among them, PACS~\cite{li2017deeper}, VLCS~\cite{fang2013unbiased}, and Office-Home~\cite{Venkateswara2017DeepHN} are three most popular datasets.
For large-scale evaluation, DomainNet~\cite{Peng2019MomentMF} and Wilds~\cite{koh2020wilds} (\emph{i.e.,} a collection of datasets in \tablename~\ref{tb-dataset} with `-wilds') are becoming popular.


Besides the datasets mentioned above, there exists some other datasets for \dg with different tasks.
The Graft-versus-host disease (GvHD) dataset~\cite{brinkman2007high} is also popular and is used to test several methods~\cite{muandet2013domain,blanchard2011generalizing} for the flow cytometry problem.
This dataset was collected from 30 patients with sample sizes ranging from 1,000 to 10,000. This is a time series classification dataset. 
Some works~\cite{gong2019dlow,yue2019domain,jin2021style} applied \dg to semantic segmentation, where CityScape~\cite{cordts2016cityscapes} and GTA5~\cite{richter2016playing} datasets were adopted as benchmark datasets.
Some works applied DG to object detection, using the datasets of Cityscapes~\cite{cordts2016cityscapes}, GTA5~\cite{richter2016playing}, Synthia~\cite{ros2016synthia} for investigation~\cite{jin2021style}.
Some other works used public datasets or RandPerson~\cite{wang2020surpassing} for person re-identification \cite{jia2019frustratingly,song2019generalizable,jin2020style}. Some works~\cite{li2018learning2,zhoudomain} used the OpenAI Gym~\cite{brockman2016openai} as the testbed to evaluate the performance of algorithms in reinforcement learning problems such as Cart-Pole and mountain car.

In addition to these widely used datasets, there are also other datasets used in existing literature.
The Parkinson’s telemonitoring dataset~\cite{little2008suitability} is popular for predicting the clinician’s motor and total UPDRS scoring of Parkinson’s disease symptoms from voice measures.
Some methods~\cite{muandet2013domain,blanchard2017domain,grubinger2015domain} used the data from several people as the training domains to learn models that generalize to unseen subjects.

% \cl{for this section, please make the orders consistent with that in applications section: images->RL->NLP for time series}

% To test \dg algorithms on a test domain, researchers often adopt the ``leave-one-domain-out'' strategy to choose one domain as the test domain and treat others as the training domains.
% It is common to split each training domain into training and validation sets, and take all validation sets for model selection and hyperparameter tuning.
% A full benchmark results of several algorithms on these image classification datasets can be found in \cite{gulrajani2021search}.

It is worth noting that the datasets of domain generalization have some overlaps with domain adaptation.
For instance, Office-31, Office-Caltech, Office-Home, and DomainNet are also widely used benchmarks for \da.
Therefore, most domain adaptation datasets can be used for \dg benchmark in addition to those we discussed here.
For example, Amazon Review dataset~\cite{blitzer2006domain} is widely used in \da. It has four different domains on product review (DVDs, Kitchen appliance, Electronics and Books), which can also be used for \dg.

\subsection{Evaluation}
To test \dg algorithm on a test domain, three strategies are proposed~\cite{gulrajani2021search}, namely, \emph{Test-domain validation set}, \emph{Leave-one-domain-out cross-validation}, and \emph{Training-domain validation set}. 
Test-domain validation set utilizes parts of the target domain as validations.
Although it can obtain the best performance in most circumstances for that validation and testing share the same distribution, there is often no access to targets when training, which means it cannot be adopted in real applications.
Leave-one-domain-out is another strategy to choose the final model when training data contains multiple sources.
It leaves one training source as the validation while treating the others as the training part.
Obviously, when only a single source exists in the training data, it is no longer applicable.
In addition, due to different distributions among sources and targets, final results rely heavily on the selections of validation, which makes final results unstable.
The most common strategy for \dg is Training-domain validation set which is used in most existing work.
In this strategy, each source is split into two parts, the training part and the validation part.
All training parts are combined for training while all validation parts are combined for selecting the best model.
Since there still exists divergences between the combined validation and the real unseen targets, this simple and most popular strategy cannot achieve the best performance for some time.

We need to mention that there may exist other evaluation protocols for DG such as \citep{ye2021towards} since designing effective evaluation protocols is often consistent with the OOD performance.
Currently, most of the works adopted the train-domain validation strategy which may not always generate good performance since the distribution of validation set is not the same as the new training data. On the other hand, using accuracy alone may not be sufficient to valid the model performance. We are looking forward to new evaluation metrics that can truly reflect the properties test distributions as much as possible in order to obtain better results.\looseness=-1

\subsection{Benchmark}
To test the performance of DG algorithms in a unified codebase, in this paper, we develop a new codebase for DG, named \emph{DeepDG}~\cite{deepdg,transferlearning.xyz}.
Compared to the existing DomainBed~\cite{gulrajani2021search}, DeepDG simplifies the data loading and model selection process, while also makes it possible to run all experiments in a single machine.
DeepDG splits the whole process into a data preparation part, a model part, a core algorithm part, a program entry, and some other auxiliary functions.
Each part can be freely modified by users without affecting other parts.
Users can add their own algorithms or datasets to DeepDG and compare with some state-of-the-art methods fairly.
The current public version of DeepDG is only for image classification and we offer supports for Office-31, PACS, VLCS, and Office-Home datasets.
Currently, nine state-of-the-art methods are implemented under the same environment, and it covers all three groups, including Data manipulation (Mixup~\cite{zhang2018mixup}), Representation learning (DDC~\cite{tzeng2014deep}, DANN~\cite{ganin2015unsupervised}, CORAL~\cite{sun2016return}), and Learning strategy (MLDG~\cite{li2018learning2}, RSC~\cite{huang2020self}, GroupDRO~\cite{sagawa2019distributionally}, ANDMask~\cite{parascandolo2020learning}).

We conduct some experiments on the two most popular image classification datasets, PACS and Office-Home, with DeepDG and \tablename~\ref{tab:my-table-deepdg} shows the results.
ResNet-18 is used as the base feature network. 
Training-domain validation set is used for selecting final models, and $20\%$ of sources are for validation while the others are for training.
From \tablename~\ref{tab:my-table-deepdg}, we observe more insightful conclusions.
(1) The baseline method, ERM, has achieved acceptable results on both datasets. Some methods, such as DANN and ANDMask, even have worse performance.
(2) Simple data augmentation method, Mixup, cannot obtain remarkable results. 
(3) CORAL has slight improvements on both datasets compared to ERM, which is consistent with results offered by DomainBed~\cite{gulrajani2021search}.
(4) RSC, a learning strategy, achieves the best performance on both datasets, but the improvements are unremarkable compared to ERM.
The results indicate the benefits of domain generalization in different tasks.


\input{tables/table_results}

==> DG survey -- TKDE/secs/sec_future.tex <==
% We summarize some future research challenges for DG.% among others.

% \subsubsection{Single-source domain generalization}
% While the mainstream DG methods focus on learning from multiple domains, for a certain application, there might be only one domain available.
% Thus, how to learn generalized models on a single domain becomes a critical challenge.
% Since the training data is limited, a possible solution is to explore more related data in other datasets to enrich the training data.
% In addition, while exploring other datasets remains expensive, we should also focus on the internal distributions inside one domain to enhance the generalization ability of a model by solving the internal domain shift.

\subsubsection{Continuous \dg}
For many real applications, a system consumes streaming data with non-stationary statistics. 
In this case, it is of great importance to perform continuous \dg that efficiently updates DG models to overcome catastrophic forgetting and adapts to new data.
While there are some \da methods focusing on continuous learning~\cite{wang2020continuously}, there are only very few investigations on continuous DG \cite{li2020sequential} whenever this is favorable in real scenarios.
%The key to this research is to design efficient online algorithms that takes less memory space for continuous update.
% Real applications are often in an online and continuous manner, i.e., the data and tasks are arriving in an online manner.
% In this case, it is of great importance to perform continuous \dg that efficiently updates DG models to overcome catastrophic forgetting and adapts to new data.
% While there are some \da methods focusing on continuous learning~\cite{wang2020continuously}, the research on DG is still not coming.
% The key to this research is to design efficient online algorithms that takes less memory space for continuous update.

\subsubsection{Domain generalization to novel categories}
The existing DG algorithms usually assume the label space for different domains are the same.
A more practical and general setting is to support the generalization on new categories, \textit{i.e.}, both domain and task generalization.
This is conceptually similar to the goal of meta-learning and zero-shot learning.
Some work~\cite{maniyar2020zero,mancini2020towards} proposed zero-shot DG and we expect more work to come in this area. There are some prior work \cite{shu2021open,zhu2021crossmatch} that tried to use the boundary-based learning paradigms or consistency regularization to solve this problem, which are good approaches that future work might build methods upon them.
% The current DG algorithms assume the label space for each domain are the same.
% While this assumption remains simple, a more practical setting should be generalizing to new categories, i.e., domain and task generalization.
% This is similar to the goal of meta-learning and zero-shot learning, but more attention should be paid on this area.
% Some initial work~\cite{maniyar2020zero} proposed zero-shot DG and we expect more work will come in this area.

\subsubsection{Interpretable domain generalization}
Disentanglement-based DG methods decompose a feature into domain-invariant/shared and domain-specific parts, which provide some interpretation to DG.
For other categories of methods, there is still a lack of deep understanding of the semantics or characteristics of learned features in DG models.
For example, how to relate the results of the approach with the input
feature space. How close are current methods to provide this level of interpretability?
Causality~\citep{liu2021learning} may be one promising tool to understand \dg networks and provide interpretations.

\subsubsection{Large-scale pre-training/self-learning and DG}
In recent years, we have witnessed the rapid development of large-scale pre-training/self-learning, such as BERT~\cite{devlin2018bert}, GPT-3~\cite{brown2020language}, and Wav2vec~\cite{baevski2020wav2vec}.
Pre-training on large-scale dataset and then finetuning the model to downstream tasks could improve its performance, where pre-training is beneficial to learn general representations. Therefore, how to design useful and efficient DG methods to help large-scale pre-training/self-learning is worth investigating. 
% Recent years have witnessed the rapid development of large-scale pre-training, such as BERT~\cite{devlin2018bert}, GPT-3~\cite{brown2020language}, and Wav2vec~\cite{baevski2020wav2vec}.
% It seems that by first pre-training on large-scale data and then finetune the model on the downstream tasks, the performance could be dramatically improved.
% Does it make DG algorithms unnecessary?
% We argue that DG is still indispensable in this situation for several reasons.
% Firstly, the pre-trained models on large datasets are based on general tasks (i.e., image classification and text classification), thus, for specific downstream tasks, the common knowledge in pre-trained datasets can only be used for initialization, while we still need DG algorithms to learn from the specific datasets.
% Secondly, even if we have pre-trained models, the downstream tasks still have domain shift issues, which depends on DG algorithms.
% Thirdly, how to take advantage of the large-scale pre-trained model to perform fast and adaptive fine-tuning is still the key problem. 

\subsubsection{Test-time Generalization}

While DG focuses on the training phase, we can also request test-time generalization in inference phase.
This further bridges \da and \dg since we can also use the inference unlabeled data for adaptation.
Very few recent works~\cite{iwasawa2021test,pandey2021domain} paid attention to this setting.
Compared to traditional DG, test-time generalization will allow more flexibility in inference time, while it requires less computation and more efficiency as there are often limited resources in inference-end devices.

\subsubsection{Performance evaluation for DG}
The recent work~\cite{gulrajani2021search} pointed out that on several datasets, the performance of some DG methods is almost the same as the baseline (i.e., ERM).
We do not take it as the full evidence that DG is not useful in real applications. Instead, we argue that this might be due to the inappropriate evaluation schemes in use today, or the domain gaps not being so large.
In more realistic situations such as person ReID where there are obvious domain gaps~\cite{jin2021style}, the improvement of DG is dramatic.
Therefore, we stay positive about the value of DG and hope researchers can also find more suitable settings and datasets for the study.

% The recent work~\cite{gulrajani2021search} pointed out that on several datasets, the performance of some DG methods is almost the same as the baseline method (i.e., empirical risk minimization).
% We do not take it as the full evidence that DG is not useful in real applications; instead, we argue that this might be due to the inappropriate evaluation schemes in current status, or the domain gaps are not so large.
% In more realistic situations such as person ReID~\cite{jin2021style}, the improvement of DG is dramatic.
% Therefore, we stay positive about the value of DG and hope researchers can also find more suitable settings and datasets for its evaluation.


==> DG survey -- TKDE/secs/sec_learn.tex <==
In addition to data manipulation and representation learning, DG was also studied in general machine learning paradigms, which is divided into several categories: \emph{ensemble learning-based DG}, \emph{meta-learning-based DG}, \emph{gradient operation-based DG}, \emph{distributionally robust optimization-based DG}, \emph{self-supervised learning-based DG}, and \emph{other strategies}.

\subsubsection{Ensemble learning-based DG}
%Ensemble is one of the most important learning paradigms in machine learning.
Ensemble learning usually combines multiple models, such as classifiers or experts, to enhance the power of models.
For \dg, ensemble learning exploits the relationship between multiple source domains by using specific network architecture designs and training strategies to improve generalization.
They assume that any sample can be regarded as an integrated sample of the multiple source domains, so the overall prediction result can be seen as the superposition of the multiple domain networks.
% Ensemble learning is the process of combining multiple models, such as classifiers or experts, to solve a particular computational intelligence problem.
% Due to the diversity of individual classifiers or models, the power of ensembles can often achieve remarkable performance.
% For \dg, ensemble learning-based methods do not focus on explicitly or implicitly reducing the domain discrepancy.
% Instead, it learns the relationship between multiple source domains by designing specific network architectures and training strategies to improve generalization.
% They assume that any sample can be regarded as an integrated feature of the multiple source domains, so the overall prediction result can be seen as the superposition of multiple domain networks.
% The optimization objective of this line of works can be formulated as:
% \begin{equation}
%     \label{eq-ensemble}
%     \min_{h} \mathbb{E}_{\mathbf{x},y}  \ell(h(\mathbf{x}),y)  + \lambda \ell_{\mathrm{relation}},
% \end{equation}
% where $\ell_{\mathrm{relation}}$ denotes the domain relation regularization, such as the learned combination weights \textit{w.r.t.} different domains.  
%to the new domains.

\citet{mancini2018best} proposed to use learnable weights for aggregating the predictions from different source specific classifiers, where a domain predictor is used to predict the probability that a sample belongs to each domain (weights). 
\citet{segu2020batch} maintained domain-dependent batch normalization (BN) statistics and BN parameters for different source domains while all the other parameters were shared. In inference, the final prediction was a linear combination of the domain-dependent models with the combination weights inferred by measuring the distances between the instance normalization statistics of the test sample and the accumulated population statistics of each domain. %weights for aggregating the predictions the batch normalization (BN) collected domain-dependent batch normalization (BN) statistics for each of the source domains. The label of a sample can be 
The work of \cite{d2018domain} proposed domain-specific layers of different source domains and learning the linear aggregation of these layers to represent a test sample.
%The work of \cite{d2018domain} extended that idea and proposed domain-specific layers to learn the linear aggregation of these layers to represent the test samples.
\citet{zhou2020domain} proposed Domain Adaptive Ensemble Learning (DAEL), where a DAEL model is composed of a CNN feature extractor shared across domains and multiple domain-specific classifier heads. Each classifier is an expert to its own domain and a non-expert to others. DAEL aims to learn these experts collaboratively, by teaching the non-experts with the expert so as to encourage the ensemble to learn how to handle data from unseen domains.
There are also other works~\cite{wu2021collaborative,dubey2021adaptive}.
Ensemble learning remains a powerful tool for DG since ensemble allows more diversity of models and features.
However, one drawback of ensemble learning-based DG is maybe its computational resources as we need more space and computations for training and saving different models.
% each trained to specialize in a particular source domain
%He \etal~\cite{he2018domain} learned different weights for different source domains on the input features, so that the input features similar to the source domains will be enhanced and the features different from all the source domains will be suppressed.

% Seg{\`u} \etal~\cite{segu2020batch} collected domain-dependent batch normalization (BN) statistics for each of the domains at training time. The label of a sample can be inferred by measuring the
% distances between the instance normalization statistics of
% the test sample and the accumulated population
% statistics of each domain.
%Then, they used such statistics to map each domains into a latent space, which they denoted as Batch Normalization Embedding (BNE).


% For this line of work, Mancini \etal~\cite{mancini2018best} proposed to use dynamic weights for aggregating multiple source domains.
% In that work, this relationship can be represented by a domain classification network to classify if a sample belongs to one of the existing domains.
% Then, it used such probabilities as confidence of domain aggregation.
% The work of \cite{d2018domain} extended that idea by using a domain-specific layer-aggregation operation to enhance the performance of integration.
% Other works~\cite{he2018domain,zhou2020domain} used domain attention block to learning domain-specific feature maps using ensemble learning.

\subsubsection{Meta-learning-based DG}
%In recent years, meta-learning~\cite{vanschoren2018meta}, or learning to learn, has gone through rapid development.
The key idea of meta-learning is to learn a general model from multiple tasks by either optimization-based methods~\cite{Finn2017ModelAgnosticMF}, metric-based learning~\cite{snell2017prototypical}, or model-based methods~\cite{santoro2016meta}.
The idea of meta-learning has been exploited for \dg. 
They divide the data form multi-source domains into meta-train and meta-test sets to simulate domain shift.
Denote $\theta$ the model parameters to be learned, meta-learning can be formulated as:
\begin{equation}
    \label{eq-meta}
    \begin{split}
    \theta^\ast &= \operatorname{Learn}(\mathcal{S}_{mte}; \phi^\ast)\\ &= \operatorname{Learn}(\mathcal{S}_{mte}; \operatorname{MetaLearn}(\mathcal{S}_{mtrn})),
    \end{split}
\end{equation}
where $\phi^\ast = \operatorname{MetaLearn}(\mathcal{S}_{mtrn})$ denotes the meta-learned parameters from the meta-train set $\mathcal{S}_{mtrn}$ which is then used to learn the model parameters $\theta^\ast$ on the meta-test set $\mathcal{S}_{mte}$.
The two functions $\operatorname{Learn}(\cdot)$ and $\operatorname{MetaLearn}(\cdot)$ are to be designed and implemented by different meta-learning algorithms, which corresponds to a bi-level optimization problem.
The gradient update can be formulated as:
\begin{equation}
    \theta = \theta - \alpha \frac{\partial (\ell(\mathcal{S}_{mte};\theta) + \beta \ell(\mathcal{S}_{mtrn};\phi))}{\partial \theta},
\end{equation}
where $\eta$ and $\beta$ are learning rates for outer and inner loops, respectively.

\citet{Finn2017ModelAgnosticMF} proposed  Model-agnostic meta-learning (MAML). Inspired by MAML, \citet{li2018learning2} proposed MLDG (meta-learning for \dg) to use the meta-learning strategy for DG.
MLDG splits the data from the source domains into meta-train and meta-test to simulate the domain shift situation to learn general representations.
%, where the model can gradually learn to adapt to the simulated test domains. Therefore, MLDG can finally learn general knowledge.
\citet{balaji2018metareg} proposed to learn a meta regularizer (MetaReg) for the classifier. \cite{li2019feature} proposed feature-critic training for the feature extractor by designing a meta optimizer.
\citet{Dou2019DomainGV} used the similar idea of MLDG and additionally introduced two complementary losses to explicitly regularize the semantic structure of feature space.
%Dou \etal~\cite{Dou2019DomainGV} proposed Model-agnostic of Semantic Features (MASF) to extend MLDG where they also perform feature alignment using semantic distribution matching.
\citet{Du2020LearningTL} proposed an extended version of information bottleneck named Meta Variational Information Bottleneck (MetaVIB).
They regularize the Kullback–Leibler (KL) divergence between distributions of latent encoding of the samples that have the same category from different domains and learn to generate weights by using stochastic neural networks.
Recently, some works also adopted meta-learning for semi-supervised DG or discriminative DG~\cite{chen2020discriminative,sharifi2020domain,wang2020meta,zhao2020learning,zhao2021learning}.
Meta-learning is widely adopted in DG research and it can be incorporated into several paradigms such as disentanglement~\cite{bui2021exploiting}.
Meta-learning performs well on massive domains since meta-learning can seek transferable knowledge from multiple tasks.

\subsubsection{Gradient operation-based DG}

Other than meta-learning and ensemble learning, several recent works consider using gradient information to force the network to learn generalized representations.
\citet{huang2020self} proposed a self-challenging training algorithm that aims to learn general representations by manipulating gradients. 
They iteratively discarded the dominant features activated on the training data, and forced the network to activate remaining features that correlate with labels. In this way, network can be forced to learn from more bad cases which will improve generalization ability.
\citet{shi2021gradient} proposed a gradient-matching scheme, where their assumption is that the gradient direction of two domains should be the same to enhance common representation learning.
To this end, they proposed to maximize the gradient inner product (GIP) to align the gradient direction
across domains. With this operation, the network can find weights such that the input-output correspondence is as close as possible
across domains. GIP can be formulated as:
\begin{equation}
    \mathcal{L}=\mathcal{L}_{\text {cls }}\left(\mathcal{S}_{t rain} ; \theta\right)-\lambda \frac{2}{M(M-1)} \sum_{i,j}^{i \neq j} G_{i} \cdot G_{j},
\end{equation}
where $G_i$ and $G_j$ are gradient for two domains that can be calulated as $G=\mathbb{E} \frac{\partial \ell(x, y; \theta)}{\partial \theta}$.
The gradient-invariance was achieved by adding CORAL~\cite{sun2016deep} loss between gradients in \cite{rame2021fishr}, while \citet{tian2021neuron} maximized the neuron coverage of
DNN with gradient similarity regularization between the
original and the augmented samples.
Additionally, \citet{wang2021embracing} designed a knowledge distillation approach for based on gradient filtering.


\subsubsection{Distributionally robust optimization-based DG}

The goal of distributionally robust optimization (DRO)~\cite{rahimian2019distributionally} is to learn a model at worst-case distribution scenario to hope it can generalize well to the test data, which shares similar goal as DG.
To optimize the worst-case distribution scenario, \citet{Sagawa2019DistributionallyRN} proposed a GroupDRO algorithm that requires explicit group annotation of the samples.
Such annotation was later narrowed down to a small fraction of validation set in \cite{liu2021just}, where they formulated a two-stage weighting framework.
Other researchers reduced the variance of training domain risks by risk extrapolation (VRex)~\cite{krueger2021out} or reducing class-conditioned Wasserstein DRO~\cite{wang2021class}.
Recently, \citet{koh2020wilds} proposed the setting of subpopulation shift where they also applied DRO to this problem.
Particularly, \citet{du2021adarnn} proposed AdaRNN, a similar algorithm to the spirit of DRO that did not require explicit group annotation; instead, they learned the worst-case distribution scenario by solving an optimization problem.
To summarize, DRO focuses on the optimization process that can also be leveraged in DG research.

\subsubsection{Self-supervised learning-based DG}

Self-supervised learning (SSL) is a recently popular learning paradigm that builds self-supervised tasks from the large-scale unlabeled data~\cite{jing2020self}.
Inspired by this, \citet{carlucci2019domain} introduced a self-supervision task of solving jigsaw puzzles to learn generalized representations.
Apart from introducing new pretext tasks, contrastive learning is another popular paradigm of self-supervised learning, which was adopted in several recent works~\cite{kim2021selfreg,li2021domain,jeon2021feature}.
The core of contrastive learning is to perform unsupervised learning between positive and negative pairs.
Note that self-supervised learning is a general paradigm that can be applied to any existing DG methods, especially unsupervised DG where there are no labels in training domains~\cite{qi2021unsupervised}.
Another possible application of SSL-based DG is the pretraining of multi-domain data that trains powerful pretraining models while also handling domain shifts.
However, a possible limitation of SSL-based DG maybe its computational efficiency and requirement of computing resources.

\subsubsection{Other learning strategy for DG}
There are some other learning strategies for \dg.
For instance, metric learning was adopted in \cite{faraki2021cross} to explore better pair-wise distance for DG.
\citet{ryu2019generalized} used random forest to improve the generalization ability of convolutional neural networks (CNN). They sampled the triplets based on the probability mass function of the split results given by random forest, which is used for updating the CNN parameters by triplet loss.
Other works~\cite{wald2021calibration,gong2021confidence} adopted model calibration for DG, where they argued that the calibrated performance has a close relationship with OOD performance.
\citet{zhang2021can} followed the lottery ticket hyphothesis to design network substructures for DG, while \citet{narayanan2021shape} focused on the shape-invariant features.
Additionally, \citet{cha2021swad} observed the flat minima is important to DG and they designed a simple stochastic weight averaging densely method to find the flat minima.
Since DG is a general learning problem, there will be more works that uses other strategy in the future.

==> DG survey -- TKDE/secs/sec_repres.tex <==
% representation learning

%The key to successful machine learning is to learn generalized representations from the training data.
Representation learning has always been the focus of machine learning for decades~\cite{bengio2013representation} and is also one of the keys to the success of \dg. 
%Therefore, apart from data manipulation methods, representation learning plays a critical role in \dg.
We decompose the prediction function $h$ as $h = f \circ g$, where $g$ is a representation learning function and $f$ is the classifier function. The goal of representation learning can be formulated as:
%We decompose the prediction function $h$ as $h = f \circ g$, where $f$ is the classifier function and $g$ is a representation learning function, then the goal of representation learning can be formulated as:
\begin{equation}
    \label{eq-repre-all}
    \min_{f,g} \, \mathbb{E}_{\mathbf{x},y}  \ell(f(g(\mathbf{x})),y)  + \lambda \ell_{\operatorname{reg}},
\end{equation}
where $\ell_{\operatorname{reg}}$ denotes some regularization term and $\lambda$ is the tradeoff parameter.
Many methods are designed to better learn the feature extraction function $g$ with corresponding $\ell_{\operatorname{reg}}$. In this section, we categorize the existing literature on representation learning into two main categories based on different learning principles: \emph{domain-invariant representation learning} and \emph{feature disentanglement}.

\subsubsection{Domain-invariant representation-based DG}

The work of \cite{ben2007analysis} theoretically proved that if the feature representations remain invariant to different domains, the representations are general and transferable to different domains (also refer to Section~\ref{sec-theory}).
%Domain-invariant representation learning originates from \da~\cite{ben2007analysis}. 
%Domain-invariant representation learning originates from \da~\cite{ben2007analysis}. Ben \etal theoretically proved that if a representation remains invariant to different domains, then the representation is general and transferable (also refer to Section~\ref{sec-theory}).
Based on this theory, a plethora of algorithms have been proposed for \da.
Similarly, for \dg, the goal is to reduce the representation discrepancy between multiple source domains in a specific feature space to be domain invariant so that the learned model can have a generalizable capability to the unseen domain. 
Along this line, there are mainly four types of methods: kernel-based methods, domain adversarial learning, explicit feature alignment, and invariant risk minimization.
%domain-invariant feature learning, 
%Similar to the \da methods, the learning goal of this type of method is to reduce the representation discrepancy between multiple source domains in a specific feature space so that the learned model can have a generalized ability to the unseen domain. 
%Along this line, there are mainly three types of methods: kernel methods, domain-invariant deep learning, and domain-adversarial learning.

\paragraph{\textbf{Kernel-based methods}}
Kernel-based method is one of the most classical learning paradigms in machine learning.
%It is worth noting that kernel based methods derive several \dg theories~\cite{blanchard2011generalizing,deshmukh2019generalization} which can be used to better analyze the methods.
Kernel-based machine learning relies on the kernel function to transform the original data into a high-dimensional feature space without ever computing the coordinates of the data in that space, but by simply computing the inner products between the samples of all pairs in the feature space.
One of the most representative kernel-based methods is Support Vector Machine (SVM)~\cite{cortes1995support}.
For \dg, there are plenty of algorithms based on kernel methods, where the representation learning function $g$ is implemented as some feature map $\phi(\cdot)$ which is easily computed using kernel function $k(\cdot, \cdot)$ such as RBF kernel and Laplacian kernel.

\citet{blanchard2011generalizing} first used kernel method for \dg  and extended it in \cite{blanchard2017domain}. They adopted the positive semi-definite kernel learning to learn a domain-invariant kernel from the training data.
%The work of \cite{blanchard2011generalizing} was the first one that used kernel method for \dg, which was then extended by the original authors in \cite{blanchard2017domain}. They adopted the positive semi-definite kernel learning to learn a domain-invariant kernel for the training data.
\citet{grubinger2015domain} adapted transfer component analysis (TCA)~\cite{Pan2011DomainAV} to bridge the multi-domain distance to be closer for DG.
Similar to the core idea of TCA, Domain-Invariant Component Analysis (DICA)~\cite{muandet2013domain} is one of the classic methods using kernel for DG.
The goal of DICA is to find a feature transformation kernel $k(\cdot, \cdot)$ that minimizes the distribution discrepancy between all data in feature space.
\citet{gan2016learning} adopted a similar method as DICA and further added attribute regularization.
In contrast to DICA which deals with the marginal distribution, \citet{li2018domain} learned a feature representation which has domain-invariant class conditional distribution.
Scatter component analysis (SCA)~\cite{ghifary2016scatter} adopted Fisher's discriminant analysis to minimize the discrepancy of representations from the same class and the same domain, and maximize the discrepancy of representations from the different classes and different domains.
\citet{erfani2016robust} proposed an Elliptical Summary Randomisation (ESRand) that comprises of a randomised kernel and elliptical data summarization.
ESRand projected each domain into an ellipse to represent the domain information and then used some similarity metric to compute the distance.
\citet{hu2019domain} proposed multi-domain discriminant analysis to perform class-wise kernel learning for DG, which is more fine-grained.
To sum up, this category of methods is often highly related to other categories to act as their divergence measures or theoretical support.

%It is worth noting that kernel based methods derive several \dg theories~\cite{blanchard2011generalizing,deshmukh2019generalization} which can be used to better analyze the methods.



\paragraph{\textbf{Domain adversarial learning}}
Domain-adversarial training is widely used for learning domain-invariant features.
\citet{ganin2015unsupervised} and \citet{Ganin2016DomainAdversarialTO} proposed Domain-adversarial neural network (DANN) for domain adaptation, which adversarially trains the generator and discriminator. The discriminator is trained to distinguish the domains while the generator is trained to fool the discriminator to learn domain invariant feature representations. 
% Domain-adversarial learning is a popular technique for domain-invariant learning.
% Originated from the GAN~\cite{goodfellow2014generative} that adversarially trains the generator and discriminator, Ganin \etal~\cite{ganin2015unsupervised,Ganin2016DomainAdversarialTO} firstly used GAN for domain adaptation and propose Domain-adversarial neural network (DANN).
% DANN adversarially trains the generator and discriminator until the discriminator cannot distinguish between the source and target domains.
\citet{Li2018DomainGW} adopted such idea for DG.
\citet{gong2019dlow} used adversarial training by gradually reducing the domain discrepancy in a manifold space.
\citet{li2018deep} proposed a conditional invariant adversarial network (CIAN) to learn class-wise adversarial networks for DG.
% Li \etal~\cite{li2018deep} proposed a conditional invariant adversarial network (CIAN) to learn class-wise adversarial networks for DG.
% Further, Li \etal~\cite{li2018domain} adapted domain adversarial training, which extended CIAN to the domain generalization setting.
Similar ideas were also used in \cite{shao2019multi,rahman2020correlation,wang2020unseen}.
\citet{jia2020single} used single-side adversarial learning and asymmetric triplet loss to make sure only the real faces from different domains were indistinguishable, but not for the fake ones. After that, the extracted features of fake faces are more dispersed than before in the feature space and those of real ones are more aggregated, leading to a better generalized class boundary for unseen domains.
%train a generalized feature extractor that can distinguish between real and fake faces.
%Jia \etal~\cite{jia2020single} used adversarial training and asymmetric triplet loss to train a generalized feature extractor that can distinguish between real and fake faces.
In addition to adversarial domain classification, \citet{zhao2020domain} introduced additional entropy regularization by minimizing the KL divergence between the conditional distributions of different training domains to push the network to learn domain-invariant features. %extended the adversarial training with
Some other GAN-based methods ~\cite{garg2020learn,sicilia2021domain,albuquerque2019adversarial} were also proposed with theoretically guaranteed generalization bound.

%Other works~\cite{garg2020learn,sicilia2021domain,albuquerque2019adversarial} developed new GAN-based methods with theoretically-guaranteed generalization bound.

%\paragraph{Domain-invariant deep learning.}
%\paragraph{Feature alignment learning.}
\paragraph{\textbf{Explicit feature alignment}}
This line of works aligns the features across source domains to learn domain-invariant representations through explicit feature distribution alignment \cite{Li2018DomainGW,Zhou2020DomainGW,peng2019moment,zhu2021self}, or feature normalization \cite{pan2018two,jia2019frustratingly,nam2018batch,jin2020style}.
\citet{motiian2017unified} introduced a cross-domain contrastive loss for representation learning, where mapped domains are semantically aligned and yet maximally separated.
%that matches the distributions in the feature space.
%Li \etal~\cite{Li2018DomainGW} explicitly minimized the feature distribution divergence in the latent space using the Maximum Mean Discrepancy (MMD)~\cite{gretton2012kernel}. They also derived an upper bound for domain-wise distribution distance that significantly reduces the computation overhead. Besides, domain adversarial training is also employed.
Some methods explicitly minimized the feature distribution divergence by minimizing the maximum mean discrepancy (MMD) \cite{tzeng2014deep,Pan2011DomainAV,wang2018visual,wang2020transfer}, second order correlation \cite{sun2016return,sun2016deep,peng2018synthetic}, both mean and variance (moment matching) \cite{peng2019moment}, Wasserstein distance \cite{Zhou2020DomainGW}, \etcno, of domains for either \da or \dg.
%Zhou \etal \cite{Zhou2020DomainGW} adopted the optimal transport with Wasserstein distance to achieve class-specific cohesion.
\citet{Zhou2020DomainGW} aligned the marginal distribution of different source domains via optimal transport by minimizing the Wasserstein distance to achieve domain-invariant feature space.

Moreover, there are some works that used feature normalization techniques to enhance domain generalization capability \cite{pan2018two,jia2019frustratingly}.
\citet{pan2018two} introduced Instance Normalization (IN) layers to CNNs to improve the generalization capability of models. IN has been extensively investigated in the field of image style transfer \cite{ulyanov2017improved,dumoulin2016learned,huang2017arbitrary}, where the style of an image is reflected by the IN parameters, \ieno, mean and variance of each feature channel. Thus, IN layers \cite{ulyanov2016instance} could be used to eliminate instance-specific style discrepancy to enhance generalization \cite{pan2018two}. However, IN is task agnostic and may remove some discriminative information. In IBNNet, IN and Batch Normalization (BN) are utilized in parallel to preserve some discriminative information \cite{pan2018two}. In \cite{nam2018batch}, BN layers are replaced by Batch-Instance Normalization (BIN) layers, which adaptively balance BN and IN for each channel by selectively using BN and IN.
\citet{jin2020style,jin2021style} proposed a Style Normalization and Restitution (SNR) module to simultaneously ensure both high generalization and discrimination capability of the networks. After the style normalization by IN, a restitution step is performed to distill task-relevant discriminative features from the residual (\ieno, the difference between the original feature and the style normalized feature) and add them back to the network to ensure high discrimination. The idea of restitution is extended to other alignment-based method to restorate helpful discriminative information dropped by alignment \cite{jin2020feature}.
Recently, \citet{qi2021unsupervised} applied IN to unsupervised DG where there are no labels in the training domains to acquire invariant and transferable features.
A combination of different normalization techniques is presented in \cite{fan2021adversarially} to show that adaptively learning the normalization technique can improve DG.
This category of methods is more flexible and can be applied to other kind of categories.

\paragraph{\textbf{Invariant risk minimization (IRM)}}
\newcommand{\clG}{\mathcal{G}}
%
\citet{arjovsky2019invariant} considered another perspective on the domain-invariance of representation for domain generalization.
They did not seek to match the representation distribution of all domains, but to enforce the optimal classifier on top of the representation space to be the same across all domains.
The intuition is that the ideal representation for prediction is the \emph{cause} of $y$, and the causal mechanism should not be affected by other factors/mechanisms, thus is domain-invariant.
Formally, IRM can be formulated as:
\begin{align}
    \min_{\substack{g \in \clG, \\
        f \in \bigcap_{i=1}^M \arg\min_{f' \in \clF} \epsilon^i (f' \circ g)}}
    \sum_{i=1}^M \epsilon^i (f \circ g)
\end{align}
for some function classes $\clF$ of $g$ and $\clF$ of $f$.
The constraint for $f$ embodies the desideratum that all domains share the same representation-level classifier, and the objective function encourages $f$ and $g$ to achieve a low source domain risk.
However, this problem is hard to solve as it involves an inner-level optimization problem in its constraint.
The authors then develop a surrogate problem to learn the feature extractor $g$ that is much more practical:
\begin{align}
    \min_{g \in \clG} \sum_{i=1}^M \epsilon^i (g) + \lambda \left\| \left. \nabla_f \epsilon^i (f \circ g) \right|_{f=1} \right\|^2,
\end{align}
where a dummy representation-level classifier $f = 1$ is considered, and the gradient norm term measures the optimality of this classifier.
The work also presents a generalization theory under a perhaps strong linear assumption, that for plenty enough source domains, the ground-truth invariant classifier can be identified.

IRM has gain notable visibility recently.
There are some further theoretical analyses on the success~\cite{pmlr-v119-ahuja20a} and failure cases of IRM~\cite{rosenfeld2020risks},
and IRM has been extended to other tasks including text classification~\cite{choe2020empirical} and reinforcement learning~\cite{sonar2020invariant}.
The idea to pursue the invariance of optimal representation-level classifier is also extended.
\citet{krueger2021out} promote this invariance by minimizing the extrapolated risk among source domains, which essentially minimizes the variance of source-domain risks.
\citet{mitrovic2021representation} aim to learn such a representation in a self-supervised setup, where the second domain is constructed by data augmentation showing various semantic-irrelevant variations.
Recently, \citet{ahuja2021invariance} found the invariance of $f$ alone is not sufficient. They found IRM still fails if $g$ captures ``fully informative invariant features'', which makes $y$ independent of $x$ on all domains. This is particularly the case for classification (vs. regression) tasks. An information bottleneck regularization is hence introduced to maintain only partially informative features.

\subsubsection{Feature disentanglement-based DG}

%In addition to aligning domain-invariant representation in the feature space, the next axis of \dg algorithms is based on disentanglement.
Disentangled representation learning aims to learn a function that maps a sample to a feature vector, which contains all the information about different factors of variation and each dimension (or a subset of dimensions) contains information about only some factor(s).
%The goal of disentangled representation learning is to learn a function that maps the observations to a low-dimensional vector that contains all the information about each factor of variation, with each coordinate (or a subset of coordinates) containing information about only one factor.
Disentanglement based DG approaches in general decompose a feature representation into understandable compositions/sub-features, with one feature being domain-shared/invariant feature and the other domain-specific feature.
%Disentanglement based domain generalization approaches aim to decompose feature representations so that we can understand the composition and function of features.
The optimization objective of disentanglement-based DG can be summarized as:
\begin{equation}
    \label{eq-disent}
    \min_{g_c, g_s, f} \mathbb{E}_{\mathbf{x},y} \ell (f(g_c(\mathbf{x})), y) + \lambda \ell_{\mathrm{reg}} + \mu \ell_{\mathrm{recon}} ([ g_c(\mathbf{x}), g_s(\mathbf{x}) ], \mathbf{x} ),
\end{equation}
where $g_c$ and $g_s$ denote the domain-shared and domain-specific feature representations, respectively.
$\lambda$ and $\mu$ are tradeoff parameters.
The loss $\ell_{\mathrm{reg}}$ is a regularization term that explicitly encourages the separation of the domain shared and specific features and $\ell_{\mathrm{recon}}$ denotes a reconstruction loss that prevents information loss.
Note that $[ g_c(\mathbf{x}), g_s(\mathbf{x}) ]$ denotes the combination of two kinds of features (which is not limited to concatenation operation).

Based on the choice of network structures and implementation mechanisms, disentanglement-based DG can mainly be categorized into three types: \emph{multi-component analysis}, \emph{generative modeling}, and \emph{causality-inspired methods}.


\paragraph{\textbf{Multi-component analysis}}
In multi-component analysis, the domain-shared and domain-specific features are in general extracted using the domain-shared and domain-specific network parameters.
%In multi-component analysis, the domain-shared and domain-specific features are extracted using the shared and specific network parameters that are manually designed.
The method of UndoBias~\cite{khosla2012undoing} started from a SVM model to maximize interval classification on all training data for \dg.
They represented the parameters of the $i$-th domain as $\mathbf{w}_i=\mathbf{w}_0+\Delta_i$, where $\mathbf{w}_0$ denotes the domain-shared parameters and $\Delta_i$ denotes the domain-specific parameters.
Some other methods extented the idea of UndoBias from different aspects.
%Some subsequent methods extented the similar starting as UndoBias in many aspects.
\citet{niu2015multi} proposed to use multi-view learning for \dg. They proposed Multi-view DG (MVDG) to learn the combination of exemplar SVMs under different views for robust generalization.
\citet{ding2017deep} designed domain-specific networks for each domain and one shared domain-invariant network for all domains to learn disentangled representations, where low-rank reconstruction is adopted to align two types of networks in structured low-rank fashion.
%which is reconstructed by low-rank .
\citet{li2017deeper} extended the idea of UndoBias into the neural network context and developed a low-rank parameterized CNN model for end-to-end training.
%Fang \etal~\cite{fang2013unbiased} utilized an unbiased measurement criterion so that it can be applied to any domains. 
\citet{zunino2020explainable} learned disentangled representations through manually comparing the attention heat maps for certain areas from different domains.
There are also other works that adopt multi-component analysis for disentanglement~\cite{deshmukh2018domain2vec,xu2014exploiting,li2017domain,piratla2020efficient,triantafillou2021learning, bui2021exploiting,kang2021dynamically,liu2021domain,peng2020domain2vec}.
In general, multi-component analysis can be implemented in different architectures and remains effective for representation disentanglement.

\paragraph{\textbf{Generative modeling}}
Generative models can be used for disentanglement from the perspective of data generation process.
%Generative model considers the problem of generalization from the data generation process in a more formative way.
This kind of methods tries to formulate the generative mechanism of the samples from the domain-level, sample-level, and label-level.
Some works further disentangle the input into class-irrelevant features, which contain the information related to specific instance~\cite{wang2021variational}.
The Domain-invariant variational autoencoder (DIVA)~\cite{ilse2019diva} disentangled the features into domain information, category information, and other information, which is learned in the VAE framework.
\citet{peng2019domain} disentangled the fine-grained domain information and category information that are learned in VAEs.
\citet{qiao2020learning} also used VAE for disentanglement, where they proposed a Unified Feature Disentanglement Network (UFDN) that treated both data domains and image attributes of interest as latent factors to be disentangled.
Similarly, \citet{zhang2021towards} disentangled the semantic and variational part of the samples.
Similar spirits also include \cite{li2021semantic,choi2021robustnet}.
\citet{nam2021reducing} proposed to disentangle the style and other information using generative models that their method is both for \da and \dg.
Generative models can not only improve OOD performance, but can also be used for generation tasks, which we believe is useful for many potential applications.

% \paragraph{\textbf{Causal inference}}
\paragraph{\textbf{Causality-inspired methods}}

Causality is a finer description of variable relations beyond statistics (joint distribution). Causal relation gives information of how the system will behave under intervention, so it is naturally suitable for transfer learning tasks, since domain shift can be seen as an intervention. Particularly, under the causal consideration, the desired representation is the true cause of the label (e.g., object shape), so that prediction will not be affected by intervention on correlated but semantically irrelevant features (e.g., background, color, style). There are a number of works~\citep{scholkopf2012causal,zhang2013domain,zhang2015multi,gong2018causal} that exploited causality for domain adaptation.

For domain generalization, \citet{he2019towards} reweighted input samples in a way to make the weighted correlation reflect causal effect. \citet{zhang2021deep} took Fourier features as the causing factors of images, and enforce the independence among these features. Using the additional data of object identity (it is a more detailed label than the class label), \citep{heinze2019conditional} enforced the conditional independence of the representation from domain index given the same object. When such object label is unavailable, \citep{Mahajan2020DomainGU} further learned an object feature based on labels in a separate stage. For single-source domain generalization, \citep{mitrovic2021representation,ouyang2021causality} used data augmentation to present information of the causal factor. The augmentation operation is seen as producing outcomes under intervention on irrelevant features, which is implemented based on specific domain knowledge.
There are also generative methods under the causal consideration. \citet{zhang2020causal} explicitly modeled a manipulation variable that causes domain shift, which may be unobserved.
% On the test domain the manipulation variable is first inferred, and prediction is made based on subsequently inferred latent representation.
\citet{liu2021learning} leveraged causal invariance for single-source generalization, i.e., the invariance of the process of generating $(x,y)$ data based on the factors, which is explained more general than inference invariance that existing methods implicitly rely on. The two factors are allowed correlated which is more realistic. They theoretically prove the identifiability of the causal factor is possible and the identification benefits generalization. \citet{sun2021recovering} extended the method and theory to multiple source domains. With more informative data, the irrelevant factor is also identifiable.

% \citet{liu2021learning} proposed a unified solution for both \da and \dg % one-shot \dg (out-of-distribution generalization) based on a causal view of data-generating process, and developed an identification guarantee for the semantic representation and generalization error bounds.
% \citet{Mahajan2020DomainGU} proposed to learn disentangled representations using causal matching where they proposed MatchDG to match inputs that are similar under the resultant representation to build an invariant classifier.


==> DG survey -- TKDE/secs/sec_research_area.tex <==
Most of the existing literature on \dg adopt the basic (traditional) definition of DG in Def.~\ref{def-dg}.
There is some existing literature that extends such setting to new scenarios to push the frontiers of DG (ref. \tablename~\ref{tb-dg-area}).
This section briefly discuss the existing DG research areas to give the readers a brief overview of this problem.

\input{tables/tb_dgarea}

\subsection{Single-source Domain Generalization}

Setting $M=1$ in Def.~\ref{def-dg} gives single-source DG.
Compared to traditional DG ($M>1$), single-source DG becomes more challenging since there are less diversity in training domains.
Thus, the key to this problem is to generate novel domains using data generation techniques to increase the diversity and informativeness of training data.
Several methods designed different generation strategies~\cite{duboudin2021encouraging,jia2020single,kim2021selfreg,li2021progressive,ouyang2021causality,peng2021out,qiao2020learning,fan2021adversarially,wang2021learningtodiversify} for single-source DG in computer vision tasks.
A recent work~\cite{du2021adarnn} studied this setting in time series data where there is usually one unified dataset by using min-max optimization.
We expect more application areas can benefit from single-source DG.

\subsection{Semi-supervised Domain Generalization}

Compared to traditional DG, semi-supervised DG does not require the full labels of training domains.
It is common to apply existing semi-supervised learning algorithms such as FixMatch~\cite{sohn2020fixmatch} and FlexMatch~\cite{zhang2021flexmatch} to learn pseudo labels for the unlabeled samples.
For instance, two recent works adopted the consistency regularization in semi-supervised learning~\cite{zhou2021semi,lin2021semi} for semi-supervised DG.
It can be seen that this setting is more general than traditional DG and we expect there will be more works in this area.



\subsection{Federated Learning with Domain Generalization}
Privacy and security of machine learning is becoming increasingly critical~\citep{zhang2022remos}.
\citet{mahajan2021connection} firstly studied this problem and showed that if the features are stable, then the model is more robust to membership inference attack.
In federated DG~\cite{yang2019federated,yang2019federatedtist}, models do not access the raw training data; instead, they aggregate the parameters from different clients.
Under this circumstance, the key is to design better aggregation scheme through generalization techniques~\cite{zhang2021federated,liu2021feddg,wu2021collaborative}.
Federated DG is more important in healthcare~\cite{chen2020fedhealth}. On the other hand, decentralized training is another possible solution~\cite{kaissis2020secure}. However, similar privacy risks emerge when there is a need to update the model. Thus, we hope there could be more research.

\subsection{Other DG Settings}

There are also other settings in DG, such as open \dg~\cite{shu2021open} and unsupervised \dg~\cite{qi2021unsupervised}.
Open DG shares the similar setting of universal domain adaptation where the training and test label spaces are not the same.
Unsupervised DG assumes that all labels in the training domains are not accessible.
As the environment gets more general and challenging, there will be other DG research areas aiming at solving certain limitations.


==> DG survey -- TKDE/secs/sec_summary.tex <==
The quantity and diversity of training data are critical to a model's generalization ability.
Many methods aim to enrich the training data with the data manipulation methods to achieve good performance.
However, one issue of the data manipulation methods is that there is a lack of theoretical guarantee of the unbound risk of generalization.
%However, one critical issue of the data manipulation methods may be the unbounded risk of generalization since the augmentation or generation methods are often not theoretically guaranteed.
Therefore, it is important to develop theories for the manipulation-based methods which could further guide the data generation designs without violating ethical standards.

Compared to data manipulation, representation learning has theoretical support in general \citep{ben2007analysis,blanchard2011generalizing,albuquerque2019adversarial}.
Kernel-based methods are widely used in traditional methods while deep learning-based methods play a leading role in recent years.
While domain adversarial training often achieves better performance in domain adaptation, in DG, we did not see significant results improvements from these adversarial methods. We think this is probably because the task is relatively easy.
For the explicit distribution matching, more and more works tend to match the joint distributions rather than just match the marginal~\citep{blanchard2011generalizing,Li2018DomainGW} or conditional~\citep{li2018domain} distributions.
Thus, it is more feasible to perform dynamic distribution matching~\citep{wang2018visual,wang2020transfer}.
Both disentanglement and IRM methods have good motivations for generalization, while more efficient training strategy can be developed.
There are several studies \cite{shui2021benefits} that pointed out merely learning domain-invariant features are insufficient and representation smoothness should also be considered.

For learning strategy, there is a trend that many works used meta-learning for DG, where it requires to design better optimization strategies to utilize the rich information of different domains.
In addition to deep networks, there are also some work~\citep{ryu2019generalized} that used random forest for DG, and we hope more diverse methods will come.

==> DG survey -- TKDE/secs/sec_theory.tex <==
\newcommand{\clA}{\mathcal{A}}
\newcommand{\clB}{\mathcal{B}}
\newcommand{\clE}{\mathcal{E}}
\newcommand{\clEh}{{\hat \clE}}
\newcommand{\clF}{\mathcal{F}}
\newcommand{\clH}{\mathcal{H}}
\newcommand{\clHt}{{\tilde \clH}}
\newcommand{\clP}{\mathcal{P}}
\newcommand{\clS}{\mathcal{S}}
\newcommand{\clU}{\mathcal{U}}
\newcommand{\clUt}{{\tilde \clU}}
\newcommand{\clX}{\mathcal{X}}
\newcommand{\clY}{\mathcal{Y}}
\newcommand{\clZ}{\mathcal{Z}}

\newcommand{\bbE}{\mathbb{E}}

\newcommand{\scX}{\mathscr{X}}

\newcommand{\frkk}{\mathfrak{k}}

\newcommand{\bfxx}{\mathbf{x}}

\newcommand{\ddh}{{\hat d}}
\newcommand{\epsilonh}{{\hat \epsilon}}

\newcommand{\kkb}{{\bar k}}

In this section, we review some theories related to \dg.
Since domain adaptation is closely related to DG, we begin with the theory of domain adaptation.
%We hope that this theoretical analysis will help researchers better analyze and understand their problems and solutions.

\subsection{Domain Adaptation}
\label{sec:thr-da}

% We begin with the theory for domain adaptation (DA).
For a binary classification problem, we denote the true labeling functions on the source domain as ${h^*}^s: \mathcal{X} \rightarrow [0,1]$
\footnote{When the output is in $(0,1)$, it means the probability of $y=1$.}
and that on the target domain as ${h^*}^t$.
%and ${h^*}^t$ on the target domain.
Let $h: \mathcal{X} \rightarrow [0,1]$ be any classifier from a hypothesis space $\clH$.
The classification difference on the source domain between two classifiers $h$ and $h'$ can then be measured by
\begin{align}
    \epsilon^s (h,h') = \bbE_{\bfxx \sim P^s_X} [h(\bfxx) \neq h'(\bfxx)] = \bbE_{\bfxx \sim P^s_X} [|h(\bfxx) - h'(\bfxx)|],
\end{align}
and similarly we can define $\epsilon^t$ when taking $\bfxx \sim P^t_X$ in the expectation.
We define $\epsilon^s(h) := \epsilon^s(h, {h^*}^s)$ and $\epsilon^t(h) := \epsilon^t(h, {h^*}^t)$ as the risk of classifier $h$ on the source and target domains, respectively.

The goal of DG/DA is to minimize the target risk $\epsilon^t(h)$, but it is not accessible since we do not have any information on ${h^*}^t$.
So people seek to bound the target risk $\epsilon^t(h)$ using the tractable source risk $\epsilon^s(h)$.
Ben-David et al. \cite{ben2010theory} (Thm.~1) give a bound relating the two risks:
\begin{align}
  \epsilon^t(h) \le{} & \epsilon^s(h) + 2 d_1(P^s_X, P^t_X) \\
  & {}+ \min_{P_X \in \{P^s_X, P^t_X\}} \bbE_{\bfxx \sim P_X} [| {h^*}^s(\bfxx) - {h^*}^t(\bfxx) |],
  \label{eqn:da-bound-tv}
\end{align}
where $d_1(P^s_X, P^t_X) := \sup_{\clA \in \scX} |P^s_X[\clA] - P^t_X[\clA]|$ is the \emph{total variation} between the two distributions, and $\scX$ denotes the sigma-field on $\clX$.
The second term on the r.h.s measures the difference of cross-domain distributions,
and the third term represents the difference in the labeling functions
(covariate shift is not \emph{a priori} assumed).
% Zhao et al. \cite{zhao2019learning} (Thm.~4.1) give a similar bound using the $\clHt$-divergence $d_\clHt (P^s_X, P^t_X) := \sup_{\clA \in \{h^{-1}(1) \mid h \in \clHt\}} |P^s_X[\clA] - P^t_X[\clA]|$,
% where $\clHt := \{\mathrm{sgn}(|h(\bfxx) - h'(\bfxx)| - t) \mid h, h' \in \clH, t \in [0, 1]\}$.

However, the total variation is a strong distance (i.e., it tends to be very large) that may loosen the bound~\eqref{eqn:da-bound-tv}, and is hard to estimate using finite samples.
To address this, \citet{ben2010theory} developed another bound (\cite{ben2010theory}, Thm.~2; \cite{johansson2019support}, Thm.~1):
\begin{align}
  \epsilon^t(h) \le{} & \epsilon^s(h) + d_{\clH\Delta\clH}(P^s_X, P^t_X) + \lambda_\clH,
  \label{eqn:da-bound-hdh}
\end{align}
where the $\clH\Delta\clH$-divergence is defined as $d_{\clH\Delta\clH}(P^s_X, P^t_X) := \sup_{h, h' \in \clH} |\epsilon^s(h, h') - \epsilon^t(h, h')|$, replacing the total variation $d_1$ to measure the distribution difference,
and the ideal joint risk $\lambda_\clH := \inf_{h \in \clH} \left[ \epsilon^s(h) + \epsilon^t(h) \right]$ measures the complexity of $\clH$ for the prediction tasks on the two domains.
$\clH\Delta\clH$-divergence has a better finite-sample guarantee, leading to a non-asymptotic bound:
\begin{theorem}[Domain adaptation error bound (non-asymptotic) \cite{ben2010theory} (Thm.~2)]
\label{the-da-nonasymp}
Let $d$ be the Vapnik–Chervonenkis (VC) dimension~\cite{vapnik1994measuring} of $\clH$, and $\clU^s$ and $\clU^t$ be unlabeled samples of size $n$ from the two domains.
Then for any $h \in \clH$ and $\delta \in (0,1)$, the following inequality holds with probability at least $1-\delta$:
\begin{align}
    \epsilon^t(h) \le{} & \epsilon^s(h) + \ddh_{\clH\Delta\clH} (\clU^s, \clU^t) + \lambda_\clH \\
    & {}+ 4 \sqrt{\frac{ 2d \log (2n) + \log (2/\delta) }{n}},
\end{align}
where $\ddh_{\clH\Delta\clH}(\clU^s, \clU^t)$ is the estimate of $d_{\clH\Delta\clH}(P^s_X, P^t_X)$ on the two sets of finite data samples.
\end{theorem}

% We start with the theory in domain adaptation that was derived by Ben-David \etal~\cite{ben2007analysis}:
In the above bounds, the domain distribution difference $d(P^s_X, P^t_X)$ is not controllable, but one may learn a representation function $g: \clX \to \clZ$ that maps the original input data $\bfxx$ to some representation space $\clZ$, so that the representation distributions of the two domains become closer.
This direction of DA is thus called DA based on domain-invariant representation (DA-DIR).
The theory of domain-invariant representations has since inspired many DA/DG methods, which can be seen in Section~\ref{sec-repr}.
% This intuition is made formal in the following theorem:
% \begin{theorem}[Domain adaptation error bound on the representation space (non-asymptotic)~\cite{ben2007analysis}]
% \label{the-da}
% Let $g: \clX \to \clZ$ be a representation function towards some representation space $\clZ$,
% and let $\clF$ denote a hypothesis space with VC dimension $d$ of classifiers on top of $\clZ$.
% For unlabeled samples $\clU^s$, $\clU^t$ of $\bfxx$ of size $n$ from the two domains, denote the samples of representations as $\clUt^s := \{g(\bfxx) \mid \bfxx \in \clU^s\}$ and $\clUt^t := \{g(\bfxx) \mid \bfxx \in \clU^t\}$.
% Then for any $f \in \clF$ and $\delta \in (0,1)$, the following inequality holds with probability at least $1-\delta$:
% \begin{align}
%     \epsilon^t(f \circ g) \le{} & \epsilonh^s(f \circ g) + \ddh_\clF (\clUt^s, \clUt^t) + \lambda_\clF \\
%     & {}+ \sqrt{\frac{4}{n} \left( d \log \frac{2n}{d} + d + \log \frac{4}{\delta} \right)},
% \end{align}
% where $\epsilonh^s(f \circ g) := \frac{1}{n} \sum_{\bfxx_j \in \clU^s} |f(g(\bfxx_j)) - {h^*}^s (\bfxx_j)|$ is the empirical source risk on the finite data samples.
% \end{theorem}

% Theorem~\ref{the-da} shows the error bound of domain adaptation on the representation space, where we can clearly see that the key to DA-DIR is to learn a proper $g$ to reduce the distribution difference between the source and target domains, i.e. $\ddh_\clF (\clUt^s, \clUt^t)$.
% which is also called the $\mathcal{H}$-divergence:
% \begin{align}
%     d_{\mathcal{H}}(\mathcal{P},\mathcal{Q}) = 2\sup\limits_{h \in \mathcal{H}}|Pr_{\mathcal{P}}[\mathbb{I}(h)] - Pr_{\mathcal{Q}}[\mathbb{I}(h)]|,
% \end{align}
% where $\mathbb{I}$ is the indicator function.



\subsection{Domain Generalization}

\subsubsection{Average risk estimation error bound}
The first line of \dg theory considers the case where the target domain is totally unknown (not even unsupervised data), and measures the average risk over all possible target domains.
Assume that all possible target distributions follow an underlying hyper-distribution $\clP$ on $(\bfxx,y)$ distributions: $P^t_{XY} \sim \clP$,
and that the source distributions also follow the same hyper-distribution: $P^1_{XY}, \cdots, P^M_{XY} \sim \clP$.
For generalization to any possible target domain, the classifier to be learned in this case also includes the domain information $P_X$ into its input, so prediction is in the form $y = h(P_X, \bfxx)$ on the domain with distribution $P_{XY}$.
For such a classifier $h$, its average risk over all possible target domains is then given by:
\begin{align}
    \clE(h) := \bbE_{P_{XY} \sim \clP} \bbE_{(\bfxx,y) \sim P_{XY}} [\ell(h(P_X, \bfxx), y)],
    \label{eqn:dg-avg-risk-exact}
\end{align}
where $\ell$ is a loss function on $\clY$.
Exactly evaluating the expectations is impossible, but we can estimate it using finite domains/distributions following $\clP$, and finite $(\bfxx,y)$ samples following each distribution.
As we have assumed $P^1_{XY}, \cdots, P^M_{XY} \sim \clP$, the source domains and supervised data could serve for this estimation:
\begin{align}
    \clEh(h) := \frac{1}{M} \sum_{i=1}^M \frac{1}{n^i} \sum_{j=1}^{n^i} \ell(h(\clU^i, \bfxx^i_j), y^i_j),
    \label{eqn:dg-avg-risk-est}
\end{align}
where we use the supervised dataset $\clU^i := \{\bfxx^i_j \mid (\bfxx^i_j, y^i_j) \in \clS^i\}$ from domain $i$ as an empirical estimation for $P^i_X$.
% \cl{in (11), $n$ was changed to $n^i$}
%where we have assumed that $n^1 = \cdots = n^M =: n$, and used the unsupervised dataset $\clU^i := \{\bfxx^i_j \mid (\bfxx^i_j, y^i_j) \in \clS^i\}$ from domain $i$ as an empirical estimation for $P^i_X$.

The first problem to consider is how well such an estimate approximates the target $\clE(h)$.
This can be measured by the largest difference between $\clE(h)$ and $\clEh(h)$ on some space of $h$.
To our knowledge, this is first analyzed by \citet{blanchard2011generalizing}, where the space of $h$ is taken as a reproducing kernel Hilbert space (RKHS).
However, different from common treatment, the classifier $h$ here also depends on the distribution $P_X$, so the kernel defining the RKHS should be in the form $\kkb((P_X^1, \bfxx_1), (P_X^2, \bfxx_2))$.
\citet{blanchard2011generalizing} construct such a kernel using kernels $k_X, k'_X$ on $\clX$ and kernel $\kappa$ on the RKHS $\clH_{k'_X}$ of kernel $k'_X$:
$\kkb((P_X^1, \bfxx_1), (P_X^2, \bfxx_2)) := \kappa(\Psi_{k'_X} (P_X^1), \Psi_{k'_X} (P_X^2)) k_X(\bfxx_1, \bfxx_2)$,
where $\Psi_{k'_X} (P_X) := \bbE_{\bfxx \sim P_X} [k'_X(\bfxx, \cdot)] \in \clH_{k'_X}$ is the kernel embedding of distribution $P_X$ via kernel $k'$.
The result is given in the following theorem, which gives a bound on the largest average risk estimation error within an origin-centered closed ball $\clB_{\clH_\kkb} (r)$ of radius $r$ in the RKHS $\clH_\kkb$ of kernel $\kkb$,
in a slightly simplified case where $n^1 = \cdots = n^M =: n$.
\begin{theorem}[Average risk estimation error bound for binary classification~\cite{blanchard2011generalizing}]
    Assume that the loss function $\ell$ is $L_\ell$-Lipschitz in its first argument and is bounded by $B_\ell$.
    Assume also that the kernels $k_X, k'_X$ and $\kappa$ are bounded by $B_k^2, B_{k'}^2 \ge 1$ and $B_\kappa^2$, respectively, and the canonical feature map $\Phi_\kappa: v \in \clH_{k'_X} \mapsto \kappa(v, \cdot) \in \clH_\kappa$ of $\kappa$ is $L_\kappa$-H\"older of order $\alpha \in (0,1]$ on the closed ball $\clB_{\clH_{k'_X}} (B_{k'})$ \footnote{
        This means that for any $u,v \in \clB_{\clH_{k'_X}} (\clB_{\clH_{k'}})$, it holds that $\Vert \Phi_\kappa(u) - \Phi_\kappa(v) \Vert \le L_\kappa \Vert u - v \Vert^\alpha$, where the norms are of the respective RKHSs.}.
    Then for any $r > 0$ and $\delta \in (0,1)$, with probability at least $1-\delta$, it holds that:
    \begin{align}
        \sup_{h \in \clB_{\clH_\kkb} (r)} \left| \clEh(h) - \clE(h) \right|
        \le{} & C \bigg( B_\ell \sqrt{- M^{-1} \log \delta} \\
        + r B_k L_\ell \Big( B_{k'} L_\kappa \big( & n^{-1} \log (M/\delta) \big)^{\alpha/2} + B_\kappa / \sqrt{M} \Big) \bigg),
    \end{align}
    where $C$ is a constant.
\end{theorem}
The bound becomes larger in general if $(M, n)$ is replaced with $(1, Mn)$.
It indicates that using domain-wise datasets is better than just pooling them into one mixed dataset, so the domain information plays a role.
This result is later extended in \cite{muandet2013domain}, and \citet{deshmukh2019generalization} give a bound for multi-class classification in a similar form.

\begin{figure*}[t!]
	\centering
	\resizebox{\textwidth}{!}{
	\input{figures/fig_tree}
	}
	\caption{Taxonomy of domain generalization methods.}
	\label{fig-main}
\end{figure*}

\subsubsection{Generalization risk bound}
% More theory: \cite{albuquerque2019adversarial,Matsuura2020DomainGU}
Another line of DG theory considers the risk on a specific target domain, under the assumption of covariate shift (i.e., the labeling function $h^*$ or $P_{Y|X}$ is the same over all domains).
This measurement is similar to what is considered in domain adaptation theory in Section~\ref{sec:thr-da}, so we adopt the same definition for the source risks $\epsilon^1, \cdots, \epsilon^M$ and the target risk $\epsilon^t$.
With the covariate shift assumption, each domain is characterized by the distribution on $\clX$.
\citet{albuquerque2019adversarial} then consider approximating the target domain distribution $P^t_X$ within the convex hull of source domain distributions: $\Lambda := \{\sum_{i=1}^M \pi_i P^i_X \mid \pi \in \Delta_M\}$, where $\Delta_M$ is the $(M-1)$-dimensional simplex so that each $\pi$ represents a normalized mixing weights.
Similar to the domain adaptation case, distribution difference is measured by the $\clH$-divergence to include the influence of the classifier class.
\begin{theorem}[Domain generalization error bound~\cite{albuquerque2019adversarial}]
    Let $\gamma := \min_{\pi \in \Delta_M} d_\clH (P^t_X, \sum_{i=1}^M \pi_i P^i_X)$ with minimizer $\pi^*$
    \footnote{The original presentation does not mention that the $\pi$ is the minimizer, but the proof indicates so.}
    be the distance of $P^t_X$ from the convex hull $\Lambda$, and $P^*_X := \sum_{i=1}^M \pi^*_i P^i_X$ be the best approximator within $\Lambda$.
    Let $\rho := \sup_{P'_X, P''_X \in \Lambda} d_\clH (P'_X, P''_X)$ be the diameter of $\Lambda$.
    Then it holds that
    \begin{align}
        \epsilon^t(h) \le \sum_{i=1}^M \pi^*_i \epsilon^i(h) + \frac{\gamma + \rho}{2} + \lambda_{\clH, (P^t_X, P^*_X)},
    \end{align}
    where $\lambda_{\clH, (P^t_X, P^*_X)}$ is the ideal joint risk across the target domain and the domain with the best approximator distribution $P^*_X$.
\end{theorem}
The result can be seen as the generalization of domain adaptation bounds in Section~\ref{sec:thr-da} when there are multiple source domains.
Again similar to the domain adaptation case, this bound motivates \dg methods based on domain invariant representation, which simultaneously minimize the risks over all source domains corresponding to the first term of the bound, as well as the representation distribution differences among source and target domains in the hope to reduce $\gamma$ and $\rho$ on the representation space.
To sum up, the theory of generalization is an active research area and other researchers also derived different DG theory bounds using informativeness~\cite{ye2021towards} and adversarial training~\cite{albuquerque2019adversarial,sicilia2021domain,ye2021towards,deshmukh2019generalization}.



\iffalse
The work of \cite{albuquerque2019adversarial} presented an adversarial learning-based DG theory:
\begin{theorem}[Domain generalization error bound~\cite{albuquerque2019adversarial,sicilia2021domain}]
\label{thm-dg-all}
Let $\mathcal{X}$ be a space and $\mathcal{H}$ be a class of hypothesis corresponding to this space. We use $\mathcal{Q}$ to denote the unseen target domain and $\{\mathcal{P}_i\}_{i=1}^{M}$ denotes the $M$ training source domains. Further, let $\{\psi_i\}_{i=1}^{M}$ denote the convex combination of the $M$ sources and $\sum_{i} \psi_i = 1$. Let the object $\mathcal{O}$ be a set of distributions such that for every distribution $\mathcal{S} \in \mathcal{O}$ the following holds:
\begin{align}
    \sum_i \psi_i d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P}_i, \mathcal{S}) \le \max_{i,j} d_{\mathcal{H} \Delta \mathcal{H}}(\mathcal{P}_i, \mathcal{P}_j).
\end{align}
Then, the following inequality holds for any $h \in \mathcal{H}$:
\begin{equation}
\begin{split}
    \epsilon_{\mathcal{Q}}(h) \le \lambda_\psi + \sum_{i} \psi_i \epsilon_{\mathcal{P}_i}(h) &+ \frac{1}{2} \min_{\mathcal{S} \in \mathcal{O}} d_{\mathcal{H} \Delta \mathcal{H}} (\mathcal{S}, \mathcal{Q})\\
    &+ \frac{1}{2} \max_{i,j} d_{\mathcal{H} \Delta \mathcal{H}} (\mathcal{P}_i, \mathcal{P}_j),
\end{split}
\end{equation}
where $\lambda_\psi = \sum_i \psi_i \lambda_i$ and each $\lambda_i$ is the error of an ideal joint hypothesis for $\mathcal{Q}$ and $\mathcal{P}_i$.
\end{theorem}
We can see that this theorem is consistent with the DA theory.
The above theorem indicates that the generalization error bound for \dg relies on four components: the ideal joint error for each source-target pair, the ERM on all source domains, the diverse joint distributions, and the source-source divergence maximization.
The third term generally inspires the data manipulation methods (Section~\ref{sec-method-data}) where some works tried to generate distributions that are near the unseen target distribution $\mathcal{Q}$.
The last term corresponds to the reduction of source-source divergence which is similar to existing DA methods. More methods can be found in Section~\ref{sec-repr}.
\fi


==> DG survey -- TKDE/tables/table_allmethods.tex <==
\begin{table*}[htbp]
\centering
\vspace{-.1in}
\caption{Summary of existing literature for \dg.}
\label{tb-all}
\vspace{-.1in}
\resizebox{.75\textwidth}{!}{
\begin{tabular}{lll}
\toprule
\textbf{Literature} & \textbf{Category} & \textbf{Application} \\ \hline
%% Data augmentation
\cite{khirodkar2019domain} & Augmentation & Car detection \\
\cite{Matsuura2020DomainGU} & Augmentation, meta-learning & Image classification \\
\cite{nazari2020domain} & Augmentation & Image classification \\
\cite{peng2018sim} & Augmentation & Reinforcement learning \\
\cite{prakash2019structured} & Augmentation & Reinforcement learning \\
CrossGrad~\cite{shankar2018generalizing} & Augmentation, adversarial & Font/Image/speech recognition \\
\cite{tobin2017domain} & Augmentation & Reinforcement learning \\
\cite{tremblay2018training} & Augmentation & Image classification \\
\cite{volpi2018generalizing} & Augmentation & Image classification \\
DomainMix~\cite{wang2020domainmix} & Augmentation & Person Re-ID \\
Mixup~\cite{wang2020heterogeneous} & Augmentation & Image classification \\
\cite{yue2019domain} & Augmentation & Image classification, semantic segmentation \\
MixStyle~\cite{zhoudomain} & Augmentation & Image classification, Person Re-ID, RL \\


%% Data generation
ADAGE~\cite{maria2019hallucinating} & Generation & Image classification \\
\cite{gulrajani2021search} & Generation & Image classification, hand pose recognition \\
DDG~\cite{rahman2019multi} & Generation & Image classification \\
\cite{somavarapu2020frustratingly} & Generation & Image classification \\
UNVP~\cite{truong2019recognition} & Generation & Image classification \\
DeGIA~\cite{truong2019image} & Generation & Image classification \\
DDAIG~\cite{zhou2020deep} & Generation & Image classification \\
L2A-OT~\cite{Zhou2020LearningTG} & Generation & Image classification \\
M-ADA~\cite{qiao2020learning} & Generation, disentangle & Image classification, semantic segmentation \\
Model-based DG~\cite{robey2021model} & Generation & Image classification \\
\hline

% Representation learning

%% Kernel method
\cite{blanchard2011generalizing} & Kernel & Flow cytometry \\
MTL~\cite{blanchard2017domain} & Kernel & Parkinson's disease, satellite image, flow cytometry \\
\cite{deshmukh2019generalization} & Kernel & Satellite image \\
ESRand~\cite{erfani2016robust} & Kernel & Activity recognition \\
KDICA~\cite{gan2016learning} & Kernel & Image classification \\
SCA~\cite{ghifary2016scatter} & Kernel & Image classification \\
TCA~\cite{grubinger2015domain} & Kernel & Landmine detection, Parkinson's disease \\
MDA~\cite{hu2019domain} & Kernel & Image classification \\
CIDDG~\cite{li2018domain} & Kernel & Image classification \\
DICA~\cite{muandet2013domain} & Kernel & Flow Cytometry, Parkinson’s disease \\


% Explicit feature alignment
\cite{ayodele2020supervised} & Explicit feature align & EEG seizure \\
\cite{chen2020study} & Explicit feature align & Image classification, physics \\
MTAE~\cite{Ghifary2015DomainGF} & Explicit feature align & Image classification \\
\cite{han2020domain} & Explicit feature align & Brain computer interface \\
SNR~\cite{jin2020style,jin2021style} & Explicit feature align & Person Re-ID, Image classification, semantic segmentation, object detection \\
FAR~\cite{jin2020feature} & Explicit feature align & Image classification \\
% FAR~\cite{jin2020feature} & Explicit feature align & Image classification, Re-ID \\
% SNR~\cite{jin2020style} & Explicit feature align & Image classification \\
\cite{li2020domain} & Explicit feature align & Fault diagnosis \\
DSDGN~\cite{liao2020deep} & Explicit feature align & Fault diagnosis \\
\cite{liu2020towards} & Explicit feature align & Water object detection \\
MatchDG~\cite{Mahajan2020DomainGU} & Explicit feature align & Image classification \\
\cite{maniyar2020zero} & Explicit feature align & Image classification \\
CCSA~\cite{motiian2017unified} & Explicit feature align & Image classification \\
BNE~\cite{segu2020batch} & Explicit feature align & Image classification \\
DSON~\cite{seo2020learning} & Explicit feature align & Image classification \\
DFDG~\cite{zhang2021robust} & Explicit feature align & Image classification \\
DDGFD~\cite{zheng2020deep} & Explicit feature align & Fault diagnosis \\
\cite{zunino2020explainable} & Explicit feature align & Image classification \\ 

% Domain adversarial learning
\cite{albuquerque2019adversarial} & Adversarial & Image classification \\
DANN~\cite{Ganin2016DomainAdversarialTO} & Adversarial & Image classification \\
DLOW~\cite{gong2019dlow} & Adversarial & Semantic segmentation \\
SSDG~\cite{jia2020single} & Adversarial & Face anti-spooﬁng \\
CIAN~\cite{li2018deep} & Adversarial & Image classification \\
MMD-AAE~\cite{Li2018DomainGW} & Adversarial & Image classification, action recognition \\
CAADG~\cite{rahman2020correlation} & Adversarial & Image classification \\
MADDG~\cite{shao2019multi} & Adversarial & Face anti-spooﬁng \\
DANNCE~\cite{sicilia2021domain} & Adversarial & Image classification \\
\cite{wang2020unseen} & Adversarial & Twitter sentence classification \\
\cite{zhao2020domain} & Adversarial & Image classification \\

%%% Invariant risk minimization
IRM~\cite{arjovsky2019invariant} & Invariant risk minimization & Image classification \\


%% Disentangle

%%% Multi-component

Domain2Vec~\cite{deshmukh2018domain2vec} & Disentangle, multi-component & Image classification \\
\cite{ding2017deep} & Disentangle, multi-component & Image classification \\
UndoBias~\cite{khosla2012undoing} & Disentangle, multi-component & Image classification \\
\cite{li2017deeper} & Disentangle, multi-component & Image classification \\
LRE~\cite{li2017domain} & Disentangle, multi-component & Image classification, action recognition \\
MVDG~\cite{niu2015multi} & Disentangle, multi-component & Image/video classification \\
CSD~\cite{piratla2020efficient} & Disentangle, multi-component & Image/speech utterance classification \\
LRE-SVM~\cite{xu2014exploiting} & Disentangle, multi-component & Image classification \\


%%% Generative modeling
DIVA~\cite{ilse2019diva} & Disentangle, generative model & Medical imaging \\
CSG~\cite{liu2020learning} & Disentangle, generative model & Image classification \\
UFDN~\cite{liu2018unified} & Disentangle, generative model & Image classification \\
DAL~\cite{peng2019domain} & Disentangle, generative model & Image classification \\
\hline

% Learning paradigm

%% Ensemble learning
D-SAM~\cite{d2018domain} & Ensemble & Image classification \\
\cite{he2018domain} & Ensemble & Human detection \\
\cite{mancini2018best} & Ensemble & Image classification \\
DAEL~\cite{zhou2020domain} & Ensemble & Image classification \\
\cite{mancini2018robust} & Ensemble & Place categorization\\

%% Meta-learning
MetaReg~\cite{balaji2018metareg} & Meta-learning & Image/sentiment classification \\
DADG~\cite{chen2020discriminative} & Meta-learning, adversarial & Image classification \\
MASF~\cite{Dou2019DomainGV} & Meta-learning & Image classification, tissue Segmentation \\
MetaVIB~\cite{Du2020LearningTL} & Meta-learning, feature align. & Image classification \\
\cite{garg2020learn} & Meta-learning & Web page classification \\
MLDG~\cite{li2018learning2} & Meta-learning & Image classification, reinforcement learning \\
Epi-FCR~\cite{li2019episodic} & Meta-learning & Image classification, action recognition \\
FC~\cite{li2019feature} & Meta-learning & Image classification \\
DGSML~\cite{sharifi2020domain} & Meta-learning, feature align & Image classification \\
\cite{wang2020meta} & Meta-learning & Semantic parsing \\
M3L~\cite{zhao2020learning} & Meta-learning & Person Re-ID \\


%% Others
Jigen~\cite{carlucci2019domain} & Self-supervision & Image classification \\
RSC~\cite{huang2020self} & Self-challenging & Image classification \\
CCFN~\cite{ryu2019generalized} & Random forest & Image classification \\
\bottomrule
\end{tabular}
}

\end{table*}





==> DG survey -- TKDE/tables/table_dataset.tex <==
\begin{table*}[t!]
  \centering
  \caption{Eighteen popular datasets for \dg. The last ten datasets are from WILDS~\cite{koh2020wilds}.}
  \label{tb-dataset}%
%   \resizebox{1\textwidth}{!}{
    \begin{tabular}{lrrrll}
    \toprule
    Dataset & \#Domain & \#Class & \#Sample & Description & Reference \\ \hline
    Office-Caltech & 4 & 10 & 2,533  & Caltech, Amazon, Webcam, DSLR & \cite{saenko2010adapting} \\
    Office-31 & 3 & 31 & 4,110  & Amazon, Webcam, DSLR & \cite{saenko2010adapting} \\
    PACS  & 4     & 7     & 9,991  & Art, Cartoon, Photos, Sketches & \cite{li2017deeper} \\
    VLCS  & 4     & 5     & 10,729  & Caltech101, LabelMe, SUN09, VOC2007 & \cite{fang2013unbiased} \\
    Office-Home & 4     & 65    & 15,588  & Art, Clipart, Product, Real & \cite{Venkateswara2017DeepHN} \\
    Terra Incognita & 4     & 10    & 24,788  & Wild animal images taken at locations L100, L38, L43, L46 & \cite{Beery2018RecognitionIT} \\
    Rotated MNIST & 6     & 10    & 70,000  & Digits rotated from $0^\circ$ to $90^\circ$ with an interval of $15^\circ$ & \cite{Ghifary2015DomainGF} \\
    DomainNet & 6     & 345   & 586,575 & Clipart, Infograph, Painting, Quickdraw, Real, Sketch & \cite{Peng2019MomentMF} \\
    iWildCam2020-wilds  & 323     & 182                                                     & 203,029 & Species classification across different   camera traps          & \cite{beery2020iwildcam}                         \\
    Camelyon17-wilds    & 5       & 2                                                       & 45,000  & Tumor identification across five different hospitals            & \cite{bandi2018detection}                        \\
    RxRx1-wilds         & 51      & 1,139                                                   & 84,898  & Genetic perturbation classification across experimental batches & \cite{taylor2019rxrx1}                           \\
    OGB-MolPCBA         & 120,084 & 128                                                     & 400,000 & Molecular property prediction across different scaffolds        & \cite{hu2020open}                                \\
    GlobalWheat-wilds   & 47      & bounding boxes     & 6,515   & Wheat head detection across regions of the world                & \cite{david2020global}          \\
    CivilComments-wilds & -       & 2                                                       & 450,000 & Toxicity classification across demographic identities           & \cite{borkan2019nuanced}                         \\
    FMoW-wilds          & 80      & 62                                                      & 118,886 & Land use classification across different regions and years      & \cite{christie2018functional}                    \\
    PovertyMap-wilds    & 46      & real value & 19,669  & Poverty mapping across different countries                      & \cite{yeh2020using}                              \\
    Amazon-wilds        & 3920    & 5                                                       & 539,502 & Sentiment classification across different users                 & \cite{ni2019justifying}                          \\
    Py150-wilds         & 8,421   & next token                                              & 150,000 & Code completion across different codebases                      & \cite{lu2021codexglue, raychev2016probabilistic}\\
    \bottomrule
    \end{tabular}
    % }
    
\end{table*}%

==> DG survey -- TKDE/tables/table_notation.tex <==
\begin{table}[htbp]
\caption{Notations used in this paper.}
\label{tb-notation}
\resizebox{.5\textwidth}{!}{
\begin{tabular}{ll|ll}
\toprule
Notation & Description & Notation & Description \\ \hline
$\mathbf{x}, y$ & Instance/label & $\ell(\cdot, \cdot)$ & Loss function \\
$\mathcal{X}, \mathcal{Y}$ & Feature/label space & $h$ & Predictive function \\ 
$\mathcal{S}$ & Domain & $g,f$ & Feature extractor/classifier \\ 
$P(\cdot)$ & Distribution & $\epsilon$ & Error (risk) \\ 
$\mathbb{E}[\cdot]$ & Expectation & $\theta$ & Model parameter \\
$M$ & Number of source domain & $n_i$ & Data size of source domain $i$ \\
\bottomrule
\end{tabular}
}
\end{table}

==> DG survey -- TKDE/tables/table_related.tex <==
\begin{table*}[t!]
\centering
\caption{Comparison between \dg and some related learning paradigms.}
\label{tb-related}
\begin{tabular}{llllc}
\toprule
Learning paradigm & Training data & Test data & Condition & Test access\\ \hline
Multi-task learning & $\mathcal{S}^1, \cdots, \mathcal{S}^n$ & $\mathcal{S}^1, \cdots, \mathcal{S}^n$ & $\mathcal{Y}^i \ne \mathcal{Y}^j, 1 \le i \ne j \le n$ & $\checkmark$\\ 
Transfer learning & $\mathcal{S}^{src}$, $\mathcal{S}^{tar}$ & $\mathcal{S}^{tar}$ & $\mathcal{Y}^{src} \ne \mathcal{Y}^{tar}$ &  $\checkmark$ \\ 
Domain adaptation & $\mathcal{S}^{src}, \mathcal{S}^{tar}$ & $\mathcal{S}^{tar}$ & $P(\mathcal{X}^{src}) \ne P(\mathcal{X}^{tar})$ &  $\checkmark$\\ 
Meta-learning & $\mathcal{S}^1, \cdots, \mathcal{S}^n$ & $\mathcal{S}^{n+1}$ & $\mathcal{Y}^i \ne \mathcal{Y}^j, 1 \le i \ne j \le n+1$ & $\checkmark$ \\ 
Lifelong learning & $\mathcal{S}^1, \cdots, \mathcal{S}^n$ & $\mathcal{S}^1, \cdots, \mathcal{S}^n$ &$\mathcal{S}^i$ arrives sequentially &$\checkmark$\\
Zero-shot learning & $\mathcal{S}^1, \cdots, \mathcal{S}^n$ & $\mathcal{S}^{n+1}$ & $\mathcal{Y}^{n+1} \ne \mathcal{Y}^i, 1 \le i \le n$ & $\times$ \\
Domain generalization & $\mathcal{S}^1, \cdots, \mathcal{S}^n$ & $\mathcal{S}^{n+1}$ & $P(\mathcal{S}^i) \ne P(\mathcal{S}^j), 1 \le i \ne j \le n+1$ & $\times$\\
\bottomrule
\end{tabular}
\vspace{-.1in}

\end{table*}

==> DG survey -- TKDE/tables/table_results.tex <==
\begin{table}[!t]
\centering
\caption{Benchmark results for PACS and Office-Home with DeepDG.}
\label{tab:my-table-deepdg}
\resizebox{.5\textwidth}{!}{
\begin{tabular}{l|ccccc|ccccc}
\toprule
Dataset  & \multicolumn{5}{c|}{PACS}              & \multicolumn{5}{c}{Office-Home}       \\
Method   & A     & C     & P     & S     & AVG   & A     & C     & P     & R     & AVG   \\
\midrule
ERM      & 77.0 & 74.5 & 95.5 & 77.8 & 81.2 & 58.6 & 47.9 & 72.2 & 73.0 & 62.9 \\
DANN~\cite{Ganin2016DomainAdversarialTO}     & 78.7 & 75.3 & 94.0 & 77.8 & 81.4 & 57.7 & 44.4 & 71.9 & 72.5  & 61.6 \\
CORAL~\cite{sun2016deep}    & 77.7 & 77.0 & 92.6 & 80.5 & 82.0 & 58.7 & 48.7 & 72.3 & 73.6 & 63.3 \\
Mixup~\cite{zhang2018mixup}    & 79.1 & 73.4 & 94.4 & 76.7 & 80.9 & 55.7 & 47.9 & 71.9 & 72.8 & 62.1 \\
RSC~\cite{huang2020self}      & 79.7 & 76.1 & 95.6 & 76.6 & 82.0 & 58.9 & 49.2 & 72.5 & 74.2 & 63.7  \\
GroupDRO~\cite{Sagawa2019DistributionallyRN} & 76.0 & 76.0 & 91.2 & 79.0 & 80.6 & 57.6  & 48.7 & 71.5 & 73.1 & 62.7 \\
ANDMask~\cite{parascandolo2020learning}  & 76.2 & 73.8 & 91.6 & 78.0 & 79.9 & 56.7 & 45.9 & 70.6 & 73.2 & 61.6 \\ \bottomrule
\end{tabular}}
\vspace{-.2in}
\end{table}

==> DG survey -- TKDE/tables/tb_dgarea.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[t!]
\centering
\caption{Existing research areas of domain generalization}
\label{tb-dg-area}
% \resizebox{.85\textwidth}{!}{%
\begin{tabular}{lll}
\toprule
Setting &
  Definition &
  Reference \\ \midrule
Traditional domain generalization &
  Def.~\ref{def-dg} &
  Most of this paper \\ 
Single-source domain generalization &
  Set $M=1$ in Def.~\ref{def-dg} &
  \cite{duboudin2021encouraging,jia2020single,kim2021selfreg,li2021progressive,ouyang2021causality,peng2021out,qiao2020learning,duboudin2021encouraging,fan2021adversarially,wang2021learningtodiversify} \\ 
Semi-supervised domain generalization &
  $\mathcal{S}_{train}$ is partially labeled &
  \cite{zhou2021semi,lin2021semi} \\ 
Federated domain generalization &
  $\mathcal{S}_{train}$ cannot broadcast to the server &
  \cite{zhang2021federated,liu2021feddg,wu2021collaborative} \\ 
Open domain generalization &
  $\mathcal{Y}_{train} \ne \mathcal{Y}_{test}$ &
  \cite{shu2021open} \\ 
Unsupervised domain generalization &
  $\mathcal{S}_{train}$ is totally unlabeled &
  \cite{qi2021unsupervised} \\ \bottomrule
\end{tabular}%
% }
\end{table*}

==> secs/sec_application_V1.0-old.tex <==
% \section{Applications}
% \label{sec-app}
In this section, we discuss popular applications for \dg.
While most of the literature utilized image classification as the main benchmark application (refer to the datasets in previous section), there are other areas where DG also plays a key role.

In computer vision, apart from image classification, satellite image classification~\cite{deshmukh2019generalization} is also a popular application for DG.
Some works also used DG for semantic segmentation~\cite{gong2019dlow}, action recognition~\cite{li2017domain,li2019episodic}, face anti-spoofing~\cite{shao2019multi}, person Re-ID~\cite{wang2020domainmix,jin2020feature}, and street view recognition~\cite{qiao2020learning}.
Also, there are some work for video understanding~\cite{niu2015multi}, and hand pose recognition~\cite{truong2019image}.
In these applications, there are also some training domains with different distributions where DG is used to learn general and robust representations.

In natural language processing, it is also common that training data comes from different domains with different distributions. 
Some work used \dg for sentiment classification on the Amazon Review dataset~\cite{wang2020unseen,balaji2018metareg}.
Others used DG for semantic parsing~\cite{wang2020meta}, web page classification~\cite{garg2020learn}.

Medical analysis is one of the key application areas for DG due to its nature of data scarcity.
In this field, tissue segmentation~\cite{Dou2019DomainGV}, Parkinson's disease~\cite{muandet2013domain}, activity recognition~\cite{erfani2016robust}, tissue segmentation~\cite{Dou2019DomainGV}, chest X-ray recognition~\cite{Mahajan2020DomainGU,li2020domain}, and EEG-based seizure detection~\cite{ayodele2020supervised}. 

Apart from those areas, DG was also used in reinforcement learning of robot control~\cite{zhoudomain,li2018learning2} to generalize to unseen environment.
Some work used DG to recognition speech utterance~\cite{shankar2018generalizing,piratla2020efficient}, fault diagnosis~\cite{li2020domain,liao2020deep,zheng2020deep}, physics~\cite{chen2020study}, brain-computer interface~\cite{han2020domain}.

Nowadays, there is a growing interest to apply existing machine learning techniques to different applications, such as financial analysis, stock prediction, weather prediction, as well as logistics.
Domain generalization is a very fundamental technology that can generally be applied to these and other areas for better generalization performance in new domains.


==> secs/sec_biography.tex <==
\begin{IEEEbiography}	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/jindwang.jpg}}]{Jindong Wang} is currently a researcher at Microsoft Research Asia, Beijing, China. He received his Ph.D. degree from Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China, in 2019. He was a visiting student in Hong Kong University of Science and Technology (HKUST) in 2018. His research interest mainly includes transfer learning, machine learning, data mining, and ubiquitous computing. He serves as the publicity co-chair of IJCAI’19 and session chair of ICDM’19. He is the reviewer or PC member of several leading journals and conferences such as TPAMI, TKDE, ICLR, ICML, NeurIPS, CVPR, etc.
\end{IEEEbiography}

\begin{IEEEbiography}	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/Cuiling_Lan.jpg}}]{Cuiling Lan} received the B.S. degree in electrical engineering and the Ph.D. degree in intelligent information processing from Xidian University, Xi’an, China, in 2008 and 2014, respectively. She joined Microsoft Research Asia, Beijing, China, in 2014. Her current research interests include computer vision problems related to pose estimation, action recognition, person/vehicle re-identification, domain generalization/adaptation.
\end{IEEEbiography}
\vspace{-3em}

\begin{IEEEbiography}	[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/ChangLiu-1}}]{Chang Liu}
is currently a researcher at Microsoft Research Asia, Machine Learning Group, starting from 2019. Before that, he received his Ph.D. degree in 2019 at the Department of Computer Science and Technology, Tsinghua University. His research interests include general Bayesian inference methods (e.g., variational inference, MCMC), Bayesian and generative modeling, and causal machine learning.

\end{IEEEbiography}
\vspace{-3em}

\begin{IEEEbiography}	[{\includegraphics[width=1in,height=1in,clip,keepaspectratio]{figures/figures_bios/yidongouyang.jpg}}]{Yidong Ouyang} is a Ph.D student in School of Data Science, Chinese University of Hong Kong, Shenzhen. His research interests include the generalization and robustness of machine learning.
\end{IEEEbiography}
\vspace{-3em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/taoqin}}]{Tao Qin}
received the Ph.D. degree and Bachelor
degree both from Tsinghua University. He is a Senior
member of ACM and IEEE, and an Adjunct Professor (Ph.D. advisor) in the University of Science
and Technology of China. He is a Senior Principal
Researcher and managing the Deep and Reinforcement Group in Microsoft Research Asia. His research interests include
machine learning (with the focus on deep learning and
reinforcement learning), artificial intelligence (with
applications to language understanding and computer
vision), game theory and multi-agent systems (with
applications to cloud computing, online and mobile advertising, ecommerce),
information retrieval and computational advertising.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/bio-wanglu}}]{Wang Lu}
received the B.S. degree in Mathematics and Applied Mathematics from Tsinghua University, Beijing, China, in 2012 and 2016, and is currently a Ph.D. candidate of the Research Center for Ubiquitous Computing Systems (CUbiCS) at the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS). His research interests include transfer learning, federated learning and activity recognition.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/yqchen.jpg}}]{Yiqiang Chen}
received the B.S. and M.S. degrees in computer science from Xiangtan University, Xiangtan, China, in 1996 and 1999, respectively, and the Ph.D. degree in computer science from the Institute of Computing Technology, Chinese Academy of Sciences, Beijing, China, in 2003. In 2004, he was a Visiting Scholar Researcher with the Department of Computer Science, Hong Kong University of Science and Technology (HKUST), Hong Kong. He is currently a professor and the director of the Pervasive Computing Research Center at the Institute of Computing Technology (ICT), Chinese Academy of Sciences (CAS). His research interests include artificial intelligence, pervasive computing, and human-computer interaction.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/Wenjun_Zeng.jpg}}]{Wenjun (Kevin) Zeng} is a Sr. Principal Research Manager and a member of the senior leadership team at Microsoft Research Asia. He was with Univ. of Missouri from 2003 to 2016, most recently as a Full Professor. Prior to that, he worked for PacketVideo Corp., Sharp Labs of America, Bell Labs, and Panasonic Technology. Wenjun has contributed significantly to the development of international standards (ISO MPEG, JPEG2000, and OMA). He received his B.E., M.S., and Ph.D. degrees from Tsinghua Univ., the Univ. of Notre Dame, and Princeton Univ., respectively. His current research interests include mobile-cloud media computing, computer vision, and multimedia communications and security.	
He is on the Editorial Board of IJCV. He was an AE of IEEE TCSVT, IEEE Trans. on Info. Forensics \& Security, and IEEE Trans. on Multimedia (TMM). He was on the Steering Committee of IEEE Trans. on Mobile Computing and IEEE TMM. He served as the Steering Committee Chair of IEEE ICME in 2010 and 2011, and has served as the General Chair or TPC Chair for several IEEE conferences ({\it e.g.}, ICME’18, ICIP’17). He was the recipient of several best paper awards. He is a Fellow of the IEEE.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/figures_bios/psyu.jpg}}]{Philip S. Yu} received the BS degree in electrical engineering from National Taiwan University, the MS and PhD degrees in electrical engineering from Stanford University, and the MBA degree from New York University. He is a distinguished professor in computer science with the University of Illinois at Chicago and also holds the Wexler chair in information technology. His research interests include big data, including data mining, data stream, database, and privacy. He has published more than 1,000 papers in refereed journals and conferences. He holds or has applied for more than 300 US patents. He is the recipient of the ACM SIGKDD 2016 Innovation Award for his influential research and scientific contributions on mining, fusion, and anonymization of big data, the IEEE Computer Society's 2013 Technical Achievement Award for pioneering and fundamentally innovative contributions to the scalable indexing, querying, searching, mining, and anonymization of big data, and the Research Contributions Award from IEEE ICDM in 2003 for his pioneering contributions to the field of data mining. He also received the ICDM 2013 10-year Highest-Impact Paper Award, and the EDBT Test of Time Award (2014). He was the editor-in-chief of the ACM Transactions on Knowledge Discovery from Data (2011-2017) and the IEEE Transactions on Knowledge and Data Engineering (2001-2004). He is a fellow of the IEEE and ACM.
\end{IEEEbiography}

==> tables/table_allmethods.tex <==
\begin{table*}[htbp]
\centering
\vspace{-.1in}
\caption{Summary of existing literature for \dg.}
\label{tb-all}
\vspace{-.1in}
\resizebox{.75\textwidth}{!}{
\begin{tabular}{lll}
\toprule
\textbf{Literature} & \textbf{Category} & \textbf{Application} \\ \hline
%% Data augmentation
\cite{khirodkar2019domain} & Augmentation & Car detection \\
\cite{Matsuura2020DomainGU} & Augmentation, meta-learning & Image classification \\
\cite{nazari2020domain} & Augmentation & Image classification \\
\cite{peng2018sim} & Augmentation & Reinforcement learning \\
\cite{prakash2019structured} & Augmentation & Reinforcement learning \\
CrossGrad~\cite{shankar2018generalizing} & Augmentation, adversarial & Font/Image/speech recognition \\
\cite{tobin2017domain} & Augmentation & Reinforcement learning \\
\cite{tremblay2018training} & Augmentation & Image classification \\
\cite{volpi2018generalizing} & Augmentation & Image classification \\
DomainMix~\cite{wang2020domainmix} & Augmentation & Person Re-ID \\
Mixup~\cite{wang2020heterogeneous} & Augmentation & Image classification \\
\cite{yue2019domain} & Augmentation & Image classification, semantic segmentation \\
MixStyle~\cite{zhoudomain} & Augmentation & Image classification, Person Re-ID, RL \\


%% Data generation
ADAGE~\cite{maria2019hallucinating} & Generation & Image classification \\
\cite{gulrajani2021search} & Generation & Image classification, hand pose recognition \\
DDG~\cite{rahman2019multi} & Generation & Image classification \\
\cite{somavarapu2020frustratingly} & Generation & Image classification \\
UNVP~\cite{truong2019recognition} & Generation & Image classification \\
DeGIA~\cite{truong2019image} & Generation & Image classification \\
DDAIG~\cite{zhou2020deep} & Generation & Image classification \\
L2A-OT~\cite{Zhou2020LearningTG} & Generation & Image classification \\
M-ADA~\cite{qiao2020learning} & Generation, disentangle & Image classification, semantic segmentation \\
Model-based DG~\cite{robey2021model} & Generation & Image classification \\
\hline

% Representation learning

%% Kernel method
\cite{blanchard2011generalizing} & Kernel & Flow cytometry \\
MTL~\cite{blanchard2017domain} & Kernel & Parkinson's disease, satellite image, flow cytometry \\
\cite{deshmukh2019generalization} & Kernel & Satellite image \\
ESRand~\cite{erfani2016robust} & Kernel & Activity recognition \\
KDICA~\cite{gan2016learning} & Kernel & Image classification \\
SCA~\cite{ghifary2016scatter} & Kernel & Image classification \\
TCA~\cite{grubinger2015domain} & Kernel & Landmine detection, Parkinson's disease \\
MDA~\cite{hu2019domain} & Kernel & Image classification \\
CIDDG~\cite{li2018domain} & Kernel & Image classification \\
DICA~\cite{muandet2013domain} & Kernel & Flow Cytometry, Parkinson’s disease \\


% Explicit feature alignment
\cite{ayodele2020supervised} & Explicit feature align & EEG seizure \\
\cite{chen2020study} & Explicit feature align & Image classification, physics \\
MTAE~\cite{Ghifary2015DomainGF} & Explicit feature align & Image classification \\
\cite{han2020domain} & Explicit feature align & Brain computer interface \\
SNR~\cite{jin2020style,jin2021style} & Explicit feature align & Person Re-ID, Image classification, semantic segmentation, object detection \\
FAR~\cite{jin2020feature} & Explicit feature align & Image classification \\
% FAR~\cite{jin2020feature} & Explicit feature align & Image classification, Re-ID \\
% SNR~\cite{jin2020style} & Explicit feature align & Image classification \\
\cite{li2020domain} & Explicit feature align & Fault diagnosis \\
DSDGN~\cite{liao2020deep} & Explicit feature align & Fault diagnosis \\
\cite{liu2020towards} & Explicit feature align & Water object detection \\
MatchDG~\cite{Mahajan2020DomainGU} & Explicit feature align & Image classification \\
\cite{maniyar2020zero} & Explicit feature align & Image classification \\
CCSA~\cite{motiian2017unified} & Explicit feature align & Image classification \\
BNE~\cite{segu2020batch} & Explicit feature align & Image classification \\
DSON~\cite{seo2020learning} & Explicit feature align & Image classification \\
DFDG~\cite{zhang2021robust} & Explicit feature align & Image classification \\
DDGFD~\cite{zheng2020deep} & Explicit feature align & Fault diagnosis \\
\cite{zunino2020explainable} & Explicit feature align & Image classification \\ 

% Domain adversarial learning
\cite{albuquerque2019adversarial} & Adversarial & Image classification \\
DANN~\cite{Ganin2016DomainAdversarialTO} & Adversarial & Image classification \\
DLOW~\cite{gong2019dlow} & Adversarial & Semantic segmentation \\
SSDG~\cite{jia2020single} & Adversarial & Face anti-spooﬁng \\
CIAN~\cite{li2018deep} & Adversarial & Image classification \\
MMD-AAE~\cite{Li2018DomainGW} & Adversarial & Image classification, action recognition \\
CAADG~\cite{rahman2020correlation} & Adversarial & Image classification \\
MADDG~\cite{shao2019multi} & Adversarial & Face anti-spooﬁng \\
DANNCE~\cite{sicilia2021domain} & Adversarial & Image classification \\
\cite{wang2020unseen} & Adversarial & Twitter sentence classification \\
\cite{zhao2020domain} & Adversarial & Image classification \\

%%% Invariant risk minimization
IRM~\cite{arjovsky2019invariant} & Invariant risk minimization & Image classification \\


%% Disentangle

%%% Multi-component

Domain2Vec~\cite{deshmukh2018domain2vec} & Disentangle, multi-component & Image classification \\
\cite{ding2017deep} & Disentangle, multi-component & Image classification \\
UndoBias~\cite{khosla2012undoing} & Disentangle, multi-component & Image classification \\
\cite{li2017deeper} & Disentangle, multi-component & Image classification \\
LRE~\cite{li2017domain} & Disentangle, multi-component & Image classification, action recognition \\
MVDG~\cite{niu2015multi} & Disentangle, multi-component & Image/video classification \\
CSD~\cite{piratla2020efficient} & Disentangle, multi-component & Image/speech utterance classification \\
LRE-SVM~\cite{xu2014exploiting} & Disentangle, multi-component & Image classification \\


%%% Generative modeling
DIVA~\cite{ilse2019diva} & Disentangle, generative model & Medical imaging \\
CSG~\cite{liu2020learning} & Disentangle, generative model & Image classification \\
UFDN~\cite{liu2018unified} & Disentangle, generative model & Image classification \\
DAL~\cite{peng2019domain} & Disentangle, generative model & Image classification \\
\hline

% Learning paradigm

%% Ensemble learning
D-SAM~\cite{d2018domain} & Ensemble & Image classification \\
\cite{he2018domain} & Ensemble & Human detection \\
\cite{mancini2018best} & Ensemble & Image classification \\
DAEL~\cite{zhou2020domain} & Ensemble & Image classification \\
\cite{mancini2018robust} & Ensemble & Place categorization\\

%% Meta-learning
MetaReg~\cite{balaji2018metareg} & Meta-learning & Image/sentiment classification \\
DADG~\cite{chen2020discriminative} & Meta-learning, adversarial & Image classification \\
MASF~\cite{Dou2019DomainGV} & Meta-learning & Image classification, tissue Segmentation \\
MetaVIB~\cite{Du2020LearningTL} & Meta-learning, feature align. & Image classification \\
\cite{garg2020learn} & Meta-learning & Web page classification \\
MLDG~\cite{li2018learning2} & Meta-learning & Image classification, reinforcement learning \\
Epi-FCR~\cite{li2019episodic} & Meta-learning & Image classification, action recognition \\
FC~\cite{li2019feature} & Meta-learning & Image classification \\
DGSML~\cite{sharifi2020domain} & Meta-learning, feature align & Image classification \\
\cite{wang2020meta} & Meta-learning & Semantic parsing \\
M3L~\cite{zhao2020learning} & Meta-learning & Person Re-ID \\


%% Others
Jigen~\cite{carlucci2019domain} & Self-supervision & Image classification \\
RSC~\cite{huang2020self} & Self-challenging & Image classification \\
CCFN~\cite{ryu2019generalized} & Random forest & Image classification \\
\bottomrule
\end{tabular}
}

\end{table*}




